CLEAR: Calibrated Learning for Epistemic and Aleatoric Risk

Accurate uncertainty quantification is critical for reliable predictive modeling. Existing methods typically address either aleatoric uncertainty due to measurement noise or epistemic uncertainty resulting from limited data, but not both in a balanced manner. We propose CLEAR, a calibration method with two distinct parameters, $\gamma_1$ and $\gamma_2$, to combine the two uncertainty components and improve the conditional coverage of predictive intervals for regression tasks. CLEAR is compatible with any pair of aleatoric and epistemic estimators; we show how it can be used with (i) quantile regression for aleatoric uncertainty and (ii) ensembles drawn from the Predictability-Computability-Stability (PCS) framework for epistemic uncertainty. Across 17 diverse real-world datasets, CLEAR achieves an average improvement of 28.3\% and 17.5\% in the interval width compared to the two individually calibrated baselines while maintaining nominal coverage. Similar improvements are observed when applying CLEAR to Deep Ensembles (epistemic) and Simultaneous Quantile Regression (aleatoric). The benefits are especially evident in scenarios dominated by high aleatoric or epistemic uncertainty. Project page: https://unco3892.github.io/clear/

==> tex_tbls/de_sqr/table-de-sqr-95-crps.tex <==
\begin{table}[!htbp]
\centering
\caption{DE-SQR CRPS at 95\% prediction intervals, aggregated across 10 seeds. CLEAR consists of the deep ensemble (DE) and the simultaneous quantile regressor (SQR). DE-conformal is the conformalized (calibrated) deep ensemble and SQR-conformal is the conformalized simultaneous quantile regressor. Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values are the minimum (best) for that dataset, while \underline{underlined} values indicate the second-best result.}
\label{tab:de_sqr_crps_95}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Dataset & CLEAR & DE & SQR & DE\text{-}conformal & SQR\text{-}conformal \\
\midrule
ailerons & \textbf{8.9e-05 $\pm$ 1.3e-06} & 1.0e-04 $\pm$ 2.1e-06 & \underline{9.0e-05 $\pm$ 1.9e-06} & 1.0e-04 $\pm$ 2.1e-06 & 9.0e-05 $\pm$ 1.3e-06 \\
airfoil & \textbf{0.873 $\pm$ 0.062} & \underline{0.936 $\pm$ 0.048} & 1.629 $\pm$ 0.164 & 0.941 $\pm$ 0.048 & 1.590 $\pm$ 0.165 \\
allstate & \textbf{1.1e+03 $\pm$ 17.709} & \underline{1.2e+03 $\pm$ 30.055} & 1.2e+03 $\pm$ 18.119 & 1.2e+03 $\pm$ 31.120 & 1.2e+03 $\pm$ 14.189 \\
ca\_housing & \textbf{2.7e+04 $\pm$ 6.0e+02} & \underline{2.9e+04 $\pm$ 6.7e+02} & 3.0e+04 $\pm$ 5.9e+02 & 2.9e+04 $\pm$ 6.7e+02 & 3.0e+04 $\pm$ 5.7e+02 \\
computer & \textbf{1.287 $\pm$ 0.017} & \underline{1.448 $\pm$ 0.043} & 1.544 $\pm$ 0.070 & 1.449 $\pm$ 0.042 & 1.547 $\pm$ 0.066 \\
concrete & \textbf{2.837 $\pm$ 0.173} & \underline{3.236 $\pm$ 0.354} & 4.340 $\pm$ 0.286 & 3.250 $\pm$ 0.356 & 4.215 $\pm$ 0.395 \\
elevator & \textbf{1.1e-03 $\pm$ 1.4e-05} & 1.3e-03 $\pm$ 1.4e-05 & \underline{1.1e-03 $\pm$ 3.4e-05} & 1.3e-03 $\pm$ 1.4e-05 & 1.1e-03 $\pm$ 3.0e-05 \\
energy\_efficiency & \textbf{0.441 $\pm$ 0.053} & \underline{0.507 $\pm$ 0.059} & 1.999 $\pm$ 0.193 & 0.515 $\pm$ 0.058 & 1.806 $\pm$ 0.224 \\
insurance & 3.7e+03 $\pm$ 4.4e+02 & \textbf{3.3e+03 $\pm$ 6.1e+02} & 3.5e+03 $\pm$ 1.8e+02 & \underline{3.5e+03 $\pm$ 6.4e+02} & 3.6e+03 $\pm$ 2.0e+02 \\
kin8nm & \textbf{0.040 $\pm$ 6.3e-04} & 0.044 $\pm$ 5.8e-04 & 0.044 $\pm$ 4.4e-04 & 0.044 $\pm$ 5.9e-04 & \underline{0.043 $\pm$ 5.9e-04} \\
miami\_housing & \textbf{3.7e+04 $\pm$ 8.5e+02} & 4.1e+04 $\pm$ 1.1e+03 & 4.0e+04 $\pm$ 1.0e+03 & 4.1e+04 $\pm$ 1.1e+03 & \underline{4.0e+04 $\pm$ 9.5e+02} \\
naval\_propulsion & \underline{5.5e-04 $\pm$ 2.1e-04} & 1.5e-03 $\pm$ 4.6e-04 & 6.4e-04 $\pm$ 3.3e-05 & 1.5e-03 $\pm$ 4.6e-04 & \textbf{4.3e-04 $\pm$ 4.2e-05} \\
parkinsons & \textbf{2.625 $\pm$ 0.057} & \underline{2.839 $\pm$ 0.079} & 3.323 $\pm$ 0.124 & 2.844 $\pm$ 0.080 & 3.317 $\pm$ 0.122 \\
powerplant & \textbf{2.053 $\pm$ 0.036} & \underline{2.332 $\pm$ 0.045} & 2.335 $\pm$ 0.039 & 2.335 $\pm$ 0.046 & 2.333 $\pm$ 0.040 \\
qsar & \textbf{0.473 $\pm$ 0.014} & \underline{0.512 $\pm$ 0.014} & 0.545 $\pm$ 0.018 & 0.512 $\pm$ 0.015 & 0.556 $\pm$ 0.016 \\
sulfur & \textbf{0.015 $\pm$ 5.2e-04} & 0.020 $\pm$ 1.2e-03 & 0.019 $\pm$ 6.5e-04 & 0.020 $\pm$ 1.2e-03 & \underline{0.019 $\pm$ 6.4e-04} \\
superconductor & \textbf{4.472 $\pm$ 0.104} & \underline{5.135 $\pm$ 0.125} & 6.168 $\pm$ 0.196 & 5.137 $\pm$ 0.126 & 6.167 $\pm$ 0.197 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/de_sqr/table-de-sqr-95-expectileloss.tex <==
\begin{table}[!htbp]
\centering
\caption{DE-SQR Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds. CLEAR consists of the deep ensemble (DE) and the simultaneous quantile regressor (SQR). DE-conformal is the conformalized (calibrated) deep ensemble and SQR-conformal is the conformalized simultaneous quantile regressor. Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values are the minimum (best) for that dataset, while \underline{underlined} values indicate the second-best result.}
\label{tab:de_sqr_expectileloss_95}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Dataset & CLEAR & DE & SQR & DE\text{-}conformal & SQR\text{-}conformal \\
\midrule
ailerons & 4.0e-09 $\pm$ 5.8e-10 & 1.1e-08 $\pm$ 6.2e-09 & \textbf{3.8e-09 $\pm$ 7.7e-10} & 1.1e-08 $\pm$ 6.2e-09 & \underline{3.9e-09 $\pm$ 6.3e-10} \\
airfoil & \textbf{0.416 $\pm$ 0.094} & \underline{0.677 $\pm$ 0.124} & 1.302 $\pm$ 0.226 & 0.684 $\pm$ 0.124 & 1.137 $\pm$ 0.208 \\
allstate & 8.5e+05 $\pm$ 1.1e+05 & 1.1e+06 $\pm$ 1.2e+05 & \textbf{7.4e+05 $\pm$ 8.0e+04} & 1.1e+06 $\pm$ 1.2e+05 & \underline{7.9e+05 $\pm$ 6.9e+04} \\
ca\_housing & \textbf{3.6e+08 $\pm$ 1.1e+07} & 7.0e+08 $\pm$ 5.1e+07 & 3.9e+08 $\pm$ 1.4e+07 & 7.0e+08 $\pm$ 5.1e+07 & \underline{3.8e+08 $\pm$ 1.0e+07} \\
computer & \textbf{0.812 $\pm$ 0.053} & \underline{1.646 $\pm$ 0.259} & 1.765 $\pm$ 0.450 & 1.651 $\pm$ 0.258 & 1.780 $\pm$ 0.419 \\
concrete & \textbf{4.619 $\pm$ 1.188} & 8.806 $\pm$ 2.449 & 9.520 $\pm$ 1.046 & 8.893 $\pm$ 2.469 & \underline{8.411 $\pm$ 1.996} \\
elevator & \textbf{5.2e-07 $\pm$ 4.4e-08} & 1.3e-06 $\pm$ 1.1e-07 & \underline{5.4e-07 $\pm$ 1.1e-07} & 1.3e-06 $\pm$ 1.1e-07 & 5.5e-07 $\pm$ 9.4e-08 \\
energy\_efficiency & \textbf{0.118 $\pm$ 0.037} & \underline{0.247 $\pm$ 0.084} & 2.247 $\pm$ 0.450 & 0.255 $\pm$ 0.085 & 1.471 $\pm$ 0.251 \\
insurance & 5.6e+06 $\pm$ 7.4e+05 & 1.0e+07 $\pm$ 5.7e+06 & \textbf{5.3e+06 $\pm$ 4.4e+05} & 1.1e+07 $\pm$ 5.9e+06 & \underline{5.6e+06 $\pm$ 1.1e+06} \\
kin8nm & \textbf{6.5e-04 $\pm$ 2.2e-05} & 1.1e-03 $\pm$ 5.5e-05 & 9.1e-04 $\pm$ 2.2e-05 & 1.2e-03 $\pm$ 5.5e-05 & \underline{7.3e-04 $\pm$ 2.6e-05} \\
miami\_housing & \textbf{1.4e+09 $\pm$ 1.5e+08} & 2.5e+09 $\pm$ 2.6e+08 & 1.4e+09 $\pm$ 9.4e+07 & 2.5e+09 $\pm$ 2.7e+08 & \underline{1.4e+09 $\pm$ 9.3e+07} \\
naval\_propulsion & \underline{1.1e-07 $\pm$ 7.9e-08} & 9.7e-07 $\pm$ 4.6e-07 & 3.0e-07 $\pm$ 2.6e-08 & 9.7e-07 $\pm$ 4.6e-07 & \textbf{9.1e-08 $\pm$ 1.7e-08} \\
parkinsons & \textbf{3.491 $\pm$ 0.204} & 5.570 $\pm$ 0.491 & 4.176 $\pm$ 0.243 & 5.603 $\pm$ 0.496 & \underline{4.014 $\pm$ 0.183} \\
powerplant & \textbf{2.063 $\pm$ 0.329} & 3.754 $\pm$ 0.400 & 2.321 $\pm$ 0.291 & 3.767 $\pm$ 0.403 & \underline{2.303 $\pm$ 0.304} \\
qsar & \underline{0.133 $\pm$ 0.028} & 0.199 $\pm$ 0.025 & \textbf{0.132 $\pm$ 0.025} & 0.199 $\pm$ 0.025 & 0.147 $\pm$ 0.023 \\
sulfur & \textbf{1.5e-04 $\pm$ 3.1e-05} & 8.3e-04 $\pm$ 2.2e-04 & 2.2e-04 $\pm$ 4.3e-05 & 8.3e-04 $\pm$ 2.2e-04 & \underline{2.2e-04 $\pm$ 4.4e-05} \\
superconductor & \textbf{15.004 $\pm$ 1.459} & 31.298 $\pm$ 2.260 & 18.358 $\pm$ 1.512 & 31.317 $\pm$ 2.262 & \underline{18.214 $\pm$ 1.481} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/de_sqr/table-de-sqr-95-mpiw.tex <==
\begin{table}[!htbp]
\centering
\caption{DE-SQR MPIW at 95\% prediction intervals, aggregated across 10 seeds. CLEAR consists of the deep ensemble (DE) and the simultaneous quantile regressor (SQR). DE-conformal is the conformalized (calibrated) deep ensemble and SQR-conformal is the conformalized simultaneous quantile regressor. Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values are the minimum (best) for that dataset, while \underline{underlined} values indicate the second-best result.}
\label{tab:de_sqr_mpiw_95}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
Dataset & CLEAR & DE & SQR & DE\text{-}conformal & SQR\text{-}conformal \\
\midrule
ailerons & \underline{6.0e-04 $\pm$ 1.4e-05} & 8.5e-04 $\pm$ 3.0e-05 & \textbf{5.9e-04 $\pm$ 3.9e-05} & 8.5e-04 $\pm$ 3.0e-05 & 6.1e-04 $\pm$ 1.4e-05 \\
airfoil & \textbf{6.336 $\pm$ 0.756} & \underline{7.612 $\pm$ 0.678} & 11.948 $\pm$ 1.111 & 7.714 $\pm$ 0.661 & 10.654 $\pm$ 1.005 \\
allstate & 8.2e+03 $\pm$ 3.6e+02 & 9.3e+03 $\pm$ 4.8e+02 & \textbf{7.0e+03 $\pm$ 4.5e+02} & 9.4e+03 $\pm$ 5.2e+02 & \underline{7.9e+03 $\pm$ 2.9e+02} \\
ca\_housing & \textbf{1.7e+05 $\pm$ 5.0e+03} & 2.4e+05 $\pm$ 1.0e+04 & 1.8e+05 $\pm$ 3.2e+03 & 2.4e+05 $\pm$ 1.0e+04 & \underline{1.8e+05 $\pm$ 2.0e+03} \\
computer & \textbf{8.574 $\pm$ 0.318} & 11.996 $\pm$ 0.624 & \underline{10.293 $\pm$ 0.881} & 12.039 $\pm$ 0.604 & 10.477 $\pm$ 0.563 \\
concrete & \textbf{20.006 $\pm$ 2.375} & \underline{27.644 $\pm$ 5.012} & 33.447 $\pm$ 2.967 & 27.972 $\pm$ 4.996 & 29.731 $\pm$ 5.041 \\
elevator & \underline{7.2e-03 $\pm$ 1.4e-04} & 0.011 $\pm$ 2.3e-04 & \textbf{7.0e-03 $\pm$ 4.0e-04} & 0.011 $\pm$ 2.3e-04 & 7.2e-03 $\pm$ 2.2e-04 \\
energy\_efficiency & \textbf{3.115 $\pm$ 0.433} & \underline{4.197 $\pm$ 0.732} & 17.484 $\pm$ 2.117 & 4.385 $\pm$ 0.729 & 13.397 $\pm$ 1.308 \\
insurance & \textbf{2.2e+04 $\pm$ 1.8e+03} & 3.0e+04 $\pm$ 8.1e+03 & \underline{2.2e+04 $\pm$ 2.4e+03} & 3.2e+04 $\pm$ 8.8e+03 & 2.3e+04 $\pm$ 4.8e+03 \\
kin8nm & \textbf{0.272 $\pm$ 6.7e-03} & 0.359 $\pm$ 9.8e-03 & 0.339 $\pm$ 5.0e-03 & 0.360 $\pm$ 1.0e-02 & \underline{0.287 $\pm$ 8.1e-03} \\
miami\_housing & \textbf{2.4e+05 $\pm$ 7.4e+03} & 3.4e+05 $\pm$ 1.4e+04 & 2.6e+05 $\pm$ 7.8e+03 & 3.4e+05 $\pm$ 1.4e+04 & \underline{2.6e+05 $\pm$ 5.2e+03} \\
naval\_propulsion & \textbf{2.7e-03 $\pm$ 7.3e-04} & 9.5e-03 $\pm$ 2.0e-03 & 6.5e-03 $\pm$ 2.3e-04 & 9.5e-03 $\pm$ 2.0e-03 & \underline{2.9e-03 $\pm$ 2.6e-04} \\
parkinsons & \textbf{18.164 $\pm$ 0.665} & 22.840 $\pm$ 1.286 & 20.101 $\pm$ 1.023 & 22.979 $\pm$ 1.308 & \underline{19.327 $\pm$ 0.824} \\
powerplant & \textbf{13.383 $\pm$ 0.272} & 19.122 $\pm$ 0.673 & 14.658 $\pm$ 0.142 & 19.191 $\pm$ 0.678 & \underline{14.528 $\pm$ 0.244} \\
qsar & \underline{3.497 $\pm$ 0.147} & 4.297 $\pm$ 0.254 & \textbf{3.425 $\pm$ 0.180} & 4.307 $\pm$ 0.256 & 3.888 $\pm$ 0.114 \\
sulfur & \textbf{0.095 $\pm$ 2.4e-03} & 0.183 $\pm$ 0.019 & 0.110 $\pm$ 4.2e-03 & 0.183 $\pm$ 0.019 & \underline{0.110 $\pm$ 3.9e-03} \\
superconductor & \textbf{29.890 $\pm$ 0.727} & 42.431 $\pm$ 1.395 & 35.664 $\pm$ 0.797 & 42.483 $\pm$ 1.406 & \underline{35.242 $\pm$ 0.689} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/de_sqr/table-sqr-de-calibration-95.tex <==
\begin{table}[!htbp]
\centering
\caption{CLEAR calibration parameters $\lambda$ and $\gamma_1$ for 95\% prediction intervals (SQR/DE benchmark). Showing mean values across runs.}
\label{tab:de_sqr_calibration_95}
\small
\begin{tabular}{lcc}
\toprule
Dataset & $\lambda$ & $\gamma_1$ \\
\midrule
ailerons & 0.155 & 1.002 \\
airfoil & 0.387 & 1.040 \\
allstate & 0.583 & 1.064 \\
ca\_housing & 0.135 & 0.958 \\
computer & 0.203 & 1.055 \\
concrete & 0.304 & 1.327 \\
elevator & 0.168 & 0.909 \\
energy\_efficiency & 0.421 & 1.230 \\
insurance & 0.121 & 1.263 \\
kin8nm & 0.155 & 1.215 \\
miami\_housing & 0.247 & 1.064 \\
naval\_propulsion & 0.000 & 0.956 \\
parkinsons & 0.368 & 1.042 \\
powerplant & 0.131 & 0.896 \\
qsar & 0.425 & 1.137 \\
sulfur & 0.157 & 0.840 \\
superconductor & 0.379 & 0.774 \\
\bottomrule
\end{tabular}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/a/table-combined-95-crps-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (a) CRPS at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_crps_95_final_conformalized_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \underline{8.6e-05 $\pm$ 7.7e-07} & 9.0e-05 $\pm$ 1.1e-06 & 8.7e-05 $\pm$ 9.8e-07 & \textbf{8.6e-05 $\pm$ 7.9e-07} \\
airfoil & 1.097 $\pm$ 0.074 & 1.115 $\pm$ 0.072 & \underline{1.095 $\pm$ 0.074} & \textbf{1.083 $\pm$ 0.062} \\
allstate & 1.1e+03 $\pm$ 36.947 & \underline{1.0e+03 $\pm$ 65.306} & \textbf{1.0e+03 $\pm$ 33.683} & 1.1e+03 $\pm$ 43.869 \\
ca\textunderscore housing & 2.6e+04 $\pm$ 2.9e+02 & \textbf{2.5e+04 $\pm$ 4.3e+02} & \underline{2.6e+04 $\pm$ 3.2e+02} & 2.6e+04 $\pm$ 4.2e+02 \\
computer & \textbf{1.354 $\pm$ 0.097} & \textcolor{red}{94.572 $\pm$ 140.866} & 1.380 $\pm$ 0.121 & \underline{1.370 $\pm$ 0.123} \\
concrete & 3.135 $\pm$ 0.293 & 3.161 $\pm$ 0.479 & \underline{2.939 $\pm$ 0.323} & \textbf{2.927 $\pm$ 0.259} \\
elevator & 1.5e-03 $\pm$ 1.4e-05 & 1.5e-03 $\pm$ 3.1e-05 & \textbf{1.4e-03 $\pm$ 9.2e-06} & \underline{1.5e-03 $\pm$ 1.3e-05} \\
energy\textunderscore efficiency & 0.296 $\pm$ 0.051 & \textcolor{red}{0.361 $\pm$ 0.036} & \textbf{0.266 $\pm$ 0.027} & \underline{0.274 $\pm$ 0.029} \\
insurance & \textcolor{red}{5.0e+03 $\pm$ 6.0e+02} & \underline{4.3e+03 $\pm$ 1.8e+03} & \textbf{3.7e+03 $\pm$ 4.9e+02} & 4.7e+03 $\pm$ 3.4e+02 \\
kin8nm & \underline{0.076 $\pm$ 0.001} & 0.077 $\pm$ 0.001 & 0.076 $\pm$ 0.001 & \textbf{0.076 $\pm$ 0.001} \\
miami\textunderscore housing & \underline{3.5e+04 $\pm$ 1.1e+03} & 3.6e+04 $\pm$ 8.9e+02 & 3.6e+04 $\pm$ 1.1e+03 & \textbf{3.4e+04 $\pm$ 9.5e+02} \\
naval\textunderscore propulsion & 1.8e-04 $\pm$ 2.1e-06 & 1.9e-04 $\pm$ 2.1e-06 & \textbf{1.8e-04 $\pm$ 2.1e-06} & \underline{1.8e-04 $\pm$ 2.0e-06} \\
parkinsons & 1.796 $\pm$ 0.073 & \textcolor{red}{2.552 $\pm$ 0.233} & \textbf{1.769 $\pm$ 0.030} & \underline{1.794 $\pm$ 0.072} \\
powerplant & \underline{1.940 $\pm$ 0.037} & 1.941 $\pm$ 0.033 & 1.984 $\pm$ 0.032 & \textbf{1.938 $\pm$ 0.034} \\
qsar & \underline{0.488 $\pm$ 0.009} & 0.500 $\pm$ 0.008 & 0.489 $\pm$ 0.009 & \textbf{0.486 $\pm$ 0.008} \\
sulfur & 0.017 $\pm$ 0.001 & 0.019 $\pm$ 0.001 & \textbf{0.016 $\pm$ 0.001} & \underline{0.017 $\pm$ 0.000} \\
superconductor & 4.571 $\pm$ 0.113 & 5.490 $\pm$ 0.120 & \underline{4.559 $\pm$ 0.115} & \textbf{4.558 $\pm$ 0.097} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/a/table-combined-95-expectileloss-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (a) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_expectileloss_95_final_conformalized_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \textbf{3.3e-09 $\pm$ 1.3e-10} & 4.3e-09 $\pm$ 1.9e-10 & 3.4e-09 $\pm$ 1.7e-10 & \underline{3.3e-09 $\pm$ 1.0e-10} \\
airfoil & \underline{0.530 $\pm$ 0.108} & 0.567 $\pm$ 0.117 & 0.567 $\pm$ 0.137 & \textbf{0.499 $\pm$ 0.071} \\
allstate & \underline{6.1e+05 $\pm$ 1.1e+05} & 6.5e+05 $\pm$ 1.7e+05 & 6.1e+05 $\pm$ 9.3e+04 & \textbf{5.8e+05 $\pm$ 9.6e+04} \\
ca\textunderscore housing & \underline{3.2e+08 $\pm$ 4.9e+06} & 3.8e+08 $\pm$ 1.2e+07 & 3.3e+08 $\pm$ 7.6e+06 & \textbf{3.2e+08 $\pm$ 6.5e+06} \\
computer & \textbf{0.903 $\pm$ 0.208} & \textcolor{red}{2.4e+04 $\pm$ 3.8e+04} & \underline{0.911 $\pm$ 0.257} & 1.064 $\pm$ 0.636 \\
concrete & 4.587 $\pm$ 0.990 & 4.680 $\pm$ 1.639 & \underline{4.243 $\pm$ 1.160} & \textbf{4.220 $\pm$ 0.866} \\
elevator & 9.2e-07 $\pm$ 4.6e-08 & \textcolor{red}{1.3e-06 $\pm$ 1.4e-07} & \textbf{8.5e-07 $\pm$ 5.6e-08} & \underline{9.1e-07 $\pm$ 4.2e-08} \\
energy\textunderscore efficiency & 0.054 $\pm$ 0.018 & \textcolor{red}{0.074 $\pm$ 0.008} & \textbf{0.041 $\pm$ 0.012} & \underline{0.044 $\pm$ 0.012} \\
insurance & 5.4e+06 $\pm$ 9.1e+05 & \textcolor{red}{2.0e+07 $\pm$ 2.1e+07} & \underline{5.2e+06 $\pm$ 1.4e+06} & \textbf{5.0e+06 $\pm$ 1.1e+06} \\
kin8nm & \underline{2.2e-03 $\pm$ 5.7e-05} & 2.3e-03 $\pm$ 6.8e-05 & 2.2e-03 $\pm$ 8.2e-05 & \textbf{2.2e-03 $\pm$ 5.4e-05} \\
miami\textunderscore housing & \underline{1.1e+09 $\pm$ 1.2e+08} & 1.3e+09 $\pm$ 1.1e+08 & 1.3e+09 $\pm$ 1.7e+08 & \textbf{1.1e+09 $\pm$ 1.1e+08} \\
naval\textunderscore propulsion & 1.0e-08 $\pm$ 1.8e-10 & \textcolor{red}{1.3e-08 $\pm$ 4.4e-10} & \textbf{9.8e-09 $\pm$ 1.7e-10} & \underline{1.0e-08 $\pm$ 1.2e-10} \\
parkinsons & \underline{1.417 $\pm$ 0.157} & \textcolor{red}{3.660 $\pm$ 0.733} & 1.645 $\pm$ 0.166 & \textbf{1.410 $\pm$ 0.156} \\
powerplant & \underline{1.923 $\pm$ 0.376} & 2.024 $\pm$ 0.338 & 2.035 $\pm$ 0.348 & \textbf{1.911 $\pm$ 0.372} \\
qsar & \underline{0.111 $\pm$ 0.028} & 0.124 $\pm$ 0.029 & 0.112 $\pm$ 0.027 & \textbf{0.110 $\pm$ 0.028} \\
sulfur & \underline{3.2e-04 $\pm$ 1.2e-04} & \textcolor{red}{4.6e-04 $\pm$ 1.7e-04} & 3.4e-04 $\pm$ 9.4e-05 & \textbf{3.0e-04 $\pm$ 1.1e-04} \\
superconductor & 13.824 $\pm$ 1.255 & \textcolor{red}{24.132 $\pm$ 1.757} & \textbf{13.053 $\pm$ 1.249} & \underline{13.708 $\pm$ 1.107} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/a/table-combined-95-gamma-lambda-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (a) CLEAR calibration parameters $\lambda$ and $\gamma_1$ for 95\% prediction intervals across 10 seeds. Using all available variables. Showing median [min:max] values.}
\label{tab:combined_gamma_lambda_95_final_conformalized_variant_a}
\small
\begin{tabular}{lccc}
\toprule
Dataset & $\lambda$ & $\gamma_1$ \\
\midrule
ailerons & 0.76 [0.50:1.70] & 1.02 [0.76:1.11] \\
airfoil & 0.38 [0.14:1.14] & 1.64 [0.84:2.66] \\
allstate & 0.10 [0.00:0.67] & 1.76 [1.27:2.02] \\
ca\textunderscore housing & 0.53 [0.39:0.67] & 1.14 [1.04:1.29] \\
computer & 0.99 [0.25:5.48] & 1.05 [0.74:1.30] \\
concrete & 3.01 [0.11:100.00] & 0.60 [0.02:3.01] \\
elevator & 3.85 [1.95:6.52] & 1.14 [0.98:1.30] \\
energy\textunderscore efficiency & 0.08 [0.00:100.00] & 2.15 [0.02:3.20] \\
insurance & 0.30 [0.00:2.17] & 1.30 [0.89:2.44] \\
kin8nm & 0.99 [0.76:1.89] & 1.08 [0.72:1.28] \\
miami\textunderscore housing & 0.38 [0.16:3.70] & 1.28 [0.37:1.64] \\
naval\textunderscore propulsion & 1.22 [0.29:1.94] & 1.20 [1.11:1.34] \\
parkinsons & 1.73 [0.75:2.17] & 0.69 [0.58:1.02] \\
powerplant & 1.87 [0.95:3.78] & 0.73 [0.43:0.93] \\
qsar & 0.97 [0.46:1.88] & 1.01 [0.77:1.44] \\
sulfur & 0.46 [0.01:4.32] & 1.31 [0.53:1.64] \\
superconductor & 0.53 [0.29:1.14] & 1.08 [0.88:1.21] \\
\bottomrule
\end{tabular}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/a/table-combined-95-mpiw-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (a) MPIW at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_mpiw_95_final_conformalized_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \textbf{5.8e-04 $\pm$ 1.3e-05} & 6.5e-04 $\pm$ 2.3e-05 & 5.8e-04 $\pm$ 1.7e-05 & \underline{5.8e-04 $\pm$ 9.3e-06} \\
airfoil & \underline{7.346 $\pm$ 0.715} & 7.438 $\pm$ 0.896 & 7.798 $\pm$ 1.239 & \textbf{7.101 $\pm$ 0.481} \\
allstate & 6.6e+03 $\pm$ 2.5e+02 & 6.5e+03 $\pm$ 8.4e+02 & \textbf{6.4e+03 $\pm$ 4.6e+02} & \underline{6.4e+03 $\pm$ 3.8e+02} \\
ca\textunderscore housing & \underline{1.6e+05 $\pm$ 3.8e+03} & 1.7e+05 $\pm$ 6.5e+03 & 1.7e+05 $\pm$ 4.7e+03 & \textbf{1.6e+05 $\pm$ 4.5e+03} \\
computer & \textbf{8.982 $\pm$ 0.636} & \textcolor{red}{7.9e+02 $\pm$ 1.2e+03} & 9.349 $\pm$ 1.583 & \underline{9.020 $\pm$ 0.752} \\
concrete & 20.614 $\pm$ 2.248 & \underline{19.706 $\pm$ 3.833} & 20.200 $\pm$ 2.955 & \textbf{18.917 $\pm$ 1.985} \\
elevator & 9.7e-03 $\pm$ 2.0e-04 & 0.011 $\pm$ 0.001 & \textbf{9.2e-03 $\pm$ 2.5e-04} & \underline{9.6e-03 $\pm$ 1.5e-04} \\
energy\textunderscore efficiency & 1.940 $\pm$ 0.324 & 2.117 $\pm$ 0.326 & \underline{1.922 $\pm$ 0.348} & \textbf{1.713 $\pm$ 0.193} \\
insurance & \underline{1.9e+04 $\pm$ 2.0e+03} & \textcolor{red}{3.1e+04 $\pm$ 1.8e+04} & 2.2e+04 $\pm$ 5.7e+03 & \textbf{1.8e+04 $\pm$ 1.6e+03} \\
kin8nm & \underline{0.500 $\pm$ 0.009} & 0.515 $\pm$ 0.011 & 0.510 $\pm$ 0.010 & \textbf{0.496 $\pm$ 0.007} \\
miami\textunderscore housing & \underline{2.2e+05 $\pm$ 7.5e+03} & 2.5e+05 $\pm$ 5.8e+03 & 2.2e+05 $\pm$ 1.3e+04 & \textbf{2.2e+05 $\pm$ 4.9e+03} \\
naval\textunderscore propulsion & 1.1e-03 $\pm$ 9.8e-06 & 1.3e-03 $\pm$ 2.8e-05 & \textbf{1.1e-03 $\pm$ 1.7e-05} & \underline{1.1e-03 $\pm$ 1.0e-05} \\
parkinsons & \textbf{10.881 $\pm$ 0.794} & \textcolor{red}{15.123 $\pm$ 1.628} & 12.136 $\pm$ 0.960 & \underline{10.917 $\pm$ 0.486} \\
powerplant & \underline{12.309 $\pm$ 0.560} & 12.897 $\pm$ 0.433 & 13.152 $\pm$ 0.343 & \textbf{12.232 $\pm$ 0.274} \\
qsar & \underline{3.145 $\pm$ 0.145} & 3.300 $\pm$ 0.115 & 3.257 $\pm$ 0.099 & \textbf{3.094 $\pm$ 0.095} \\
sulfur & 0.102 $\pm$ 0.003 & 0.124 $\pm$ 0.008 & \textbf{0.098 $\pm$ 0.004} & \underline{0.099 $\pm$ 0.004} \\
superconductor & 28.456 $\pm$ 0.884 & 35.742 $\pm$ 1.250 & \textbf{28.155 $\pm$ 0.880} & \underline{28.172 $\pm$ 0.513} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/a/table-uncertainty-metrics-95_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (a) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_conformalized_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.42 [0.28:0.94] \\
airfoil & 4.24 [2.33:6.69] & 2.81 [1.60:4.77] & 0.70 [0.24:2.04] \\
allstate & 6242.71 [4418.03:6942.61] & 444.97 [0.00:2020.38] & 0.07 [0.00:0.46] \\
ca\textunderscore housing & 124233.23 [116128.73:140499.66] & 36688.78 [30210.52:42274.41] & 0.29 [0.22:0.36] \\
computer & 6.28 [4.38:7.85] & 2.55 [0.82:6.25] & 0.42 [0.10:1.43] \\
concrete & 5.57 [0.08:17.11] & 16.37 [3.89:18.84] & 3.98 [0.23:217.70] \\
elevator & 0.01 [0.01:0.01] & 0.00 [0.00:0.00] & 0.40 [0.19:0.64] \\
energy\textunderscore efficiency & 1.41 [0.01:1.78] & 0.32 [0.00:2.68] & 0.21 [0.00:256.94] \\
insurance & 16769.91 [12797.73:19012.42] & 1783.86 [0.00:8787.67] & 0.10 [0.00:0.55] \\
kin8nm & 0.23 [0.16:0.27] & 0.27 [0.23:0.35] & 1.16 [0.88:2.17] \\
miami\textunderscore housing & 147841.18 [42132.61:190207.05] & 66143.03 [37463.58:185821.66] & 0.44 [0.20:4.41] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.18 [0.04:0.29] \\
parkinsons & 5.88 [4.91:8.72] & 5.10 [3.03:6.00] & 0.90 [0.41:1.11] \\
powerplant & 5.84 [3.51:7.53] & 6.89 [4.53:8.31] & 1.17 [0.60:2.37] \\
qsar & 1.63 [1.27:2.31] & 1.42 [0.96:2.10] & 0.87 [0.42:1.65] \\
sulfur & 0.08 [0.03:0.10] & 0.02 [0.00:0.07] & 0.19 [0.01:2.25] \\
superconductor & 22.93 [18.62:25.34] & 5.62 [3.35:9.70] & 0.24 [0.13:0.52] \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/b/table-combined-95-crps-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (b) CRPS at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_crps_95_final_conformalized_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \underline{8.6e-05 $\pm$ 7.7e-07} & 9.0e-05 $\pm$ 1.1e-06 & 8.7e-05 $\pm$ 9.8e-07 & \textbf{8.6e-05 $\pm$ 7.9e-07} \\
airfoil & 1.097 $\pm$ 0.074 & 1.115 $\pm$ 0.072 & \underline{1.095 $\pm$ 0.074} & \textbf{1.083 $\pm$ 0.062} \\
allstate & 1.0e+03 $\pm$ 32.628 & \underline{1.0e+03 $\pm$ 39.579} & \textbf{1.0e+03 $\pm$ 34.276} & 1.1e+03 $\pm$ 31.229 \\
ca\textunderscore housing & 2.6e+04 $\pm$ 2.9e+02 & \textbf{2.5e+04 $\pm$ 4.3e+02} & \underline{2.6e+04 $\pm$ 3.2e+02} & 2.6e+04 $\pm$ 4.2e+02 \\
computer & \underline{1.556 $\pm$ 0.070} & 2.003 $\pm$ 0.102 & \textbf{1.540 $\pm$ 0.047} & 1.559 $\pm$ 0.073 \\
concrete & 3.024 $\pm$ 0.234 & 2.975 $\pm$ 0.312 & \textbf{2.863 $\pm$ 0.313} & \underline{2.927 $\pm$ 0.259} \\
elevator & \textbf{1.3e-03 $\pm$ 1.6e-05} & 1.5e-03 $\pm$ 3.5e-05 & 1.4e-03 $\pm$ 1.9e-05 & \underline{1.3e-03 $\pm$ 1.3e-05} \\
energy\textunderscore efficiency & 0.296 $\pm$ 0.051 & \textcolor{red}{0.361 $\pm$ 0.036} & \textbf{0.266 $\pm$ 0.027} & \underline{0.274 $\pm$ 0.029} \\
insurance & \textcolor{red}{5.5e+03 $\pm$ 6.1e+02} & \underline{4.3e+03 $\pm$ 2.0e+03} & \textbf{3.2e+03 $\pm$ 2.6e+02} & \textcolor{red}{5.2e+03 $\pm$ 7.0e+02} \\
kin8nm & \underline{0.076 $\pm$ 0.001} & 0.077 $\pm$ 0.001 & 0.076 $\pm$ 0.001 & \textbf{0.076 $\pm$ 0.001} \\
miami\textunderscore housing & \underline{3.5e+04 $\pm$ 1.1e+03} & 3.6e+04 $\pm$ 8.9e+02 & 3.6e+04 $\pm$ 1.1e+03 & \textbf{3.4e+04 $\pm$ 9.5e+02} \\
naval\textunderscore propulsion & \textbf{5.0e-04 $\pm$ 1.7e-05} & \textcolor{red}{1.9e-03 $\pm$ 1.2e-04} & 5.1e-04 $\pm$ 1.7e-05 & \underline{5.0e-04 $\pm$ 1.9e-05} \\
parkinsons & \underline{2.164 $\pm$ 0.055} & 2.424 $\pm$ 0.038 & \textbf{2.162 $\pm$ 0.053} & 2.166 $\pm$ 0.048 \\
powerplant & \underline{1.940 $\pm$ 0.037} & 1.941 $\pm$ 0.033 & 1.984 $\pm$ 0.032 & \textbf{1.938 $\pm$ 0.034} \\
qsar & \underline{0.488 $\pm$ 0.008} & 0.504 $\pm$ 0.008 & 0.491 $\pm$ 0.010 & \textbf{0.487 $\pm$ 0.008} \\
sulfur & 0.017 $\pm$ 0.001 & 0.018 $\pm$ 0.000 & \textbf{0.016 $\pm$ 0.000} & \underline{0.017 $\pm$ 0.000} \\
superconductor & \underline{5.296 $\pm$ 0.137} & 5.379 $\pm$ 0.132 & 5.382 $\pm$ 0.132 & \textbf{5.285 $\pm$ 0.152} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/b/table-combined-95-expectileloss-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (b) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_expectileloss_95_final_conformalized_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \textbf{3.3e-09 $\pm$ 1.3e-10} & 4.3e-09 $\pm$ 1.9e-10 & 3.4e-09 $\pm$ 1.7e-10 & \underline{3.3e-09 $\pm$ 1.0e-10} \\
airfoil & \underline{0.530 $\pm$ 0.108} & 0.567 $\pm$ 0.117 & 0.567 $\pm$ 0.137 & \textbf{0.499 $\pm$ 0.071} \\
allstate & \underline{5.8e+05 $\pm$ 6.5e+04} & 6.2e+05 $\pm$ 8.1e+04 & 6.1e+05 $\pm$ 8.3e+04 & \textbf{5.8e+05 $\pm$ 7.1e+04} \\
ca\textunderscore housing & \underline{3.2e+08 $\pm$ 4.9e+06} & 3.8e+08 $\pm$ 1.2e+07 & 3.3e+08 $\pm$ 7.6e+06 & \textbf{3.2e+08 $\pm$ 6.5e+06} \\
computer & \textbf{1.376 $\pm$ 0.221} & \textcolor{red}{4.389 $\pm$ 0.585} & 1.590 $\pm$ 0.251 & \underline{1.387 $\pm$ 0.244} \\
concrete & 4.498 $\pm$ 0.849 & \textbf{4.143 $\pm$ 1.108} & 4.403 $\pm$ 1.219 & \underline{4.220 $\pm$ 0.866} \\
elevator & \textbf{8.1e-07 $\pm$ 3.4e-08} & \textcolor{red}{1.6e-06 $\pm$ 1.2e-07} & 9.1e-07 $\pm$ 5.7e-08 & \underline{8.1e-07 $\pm$ 3.7e-08} \\
energy\textunderscore efficiency & 0.054 $\pm$ 0.018 & \textcolor{red}{0.074 $\pm$ 0.008} & \textbf{0.041 $\pm$ 0.012} & \underline{0.044 $\pm$ 0.012} \\
insurance & 5.4e+06 $\pm$ 9.5e+05 & \textcolor{red}{1.4e+07 $\pm$ 1.3e+07} & \underline{5.1e+06 $\pm$ 1.7e+06} & \textbf{5.0e+06 $\pm$ 9.8e+05} \\
kin8nm & \underline{2.2e-03 $\pm$ 5.7e-05} & 2.3e-03 $\pm$ 6.8e-05 & 2.2e-03 $\pm$ 8.2e-05 & \textbf{2.2e-03 $\pm$ 5.4e-05} \\
miami\textunderscore housing & \underline{1.1e+09 $\pm$ 1.2e+08} & 1.3e+09 $\pm$ 1.1e+08 & 1.3e+09 $\pm$ 1.7e+08 & \textbf{1.1e+09 $\pm$ 1.1e+08} \\
naval\textunderscore propulsion & \underline{1.4e-07 $\pm$ 1.7e-08} & \textcolor{red}{4.1e-06 $\pm$ 4.4e-07} & 1.5e-07 $\pm$ 1.8e-08 & \textbf{1.4e-07 $\pm$ 1.8e-08} \\
parkinsons & \textbf{1.769 $\pm$ 0.110} & \textcolor{red}{2.378 $\pm$ 0.176} & 1.915 $\pm$ 0.114 & \underline{1.782 $\pm$ 0.081} \\
powerplant & \underline{1.923 $\pm$ 0.376} & 2.024 $\pm$ 0.338 & 2.035 $\pm$ 0.348 & \textbf{1.911 $\pm$ 0.372} \\
qsar & \underline{0.111 $\pm$ 0.026} & 0.127 $\pm$ 0.029 & 0.113 $\pm$ 0.027 & \textbf{0.110 $\pm$ 0.027} \\
sulfur & \underline{2.6e-04 $\pm$ 3.7e-05} & \textcolor{red}{3.8e-04 $\pm$ 4.2e-05} & 3.2e-04 $\pm$ 5.4e-05 & \textbf{2.6e-04 $\pm$ 3.9e-05} \\
superconductor & 15.757 $\pm$ 1.348 & 19.503 $\pm$ 1.794 & \underline{15.676 $\pm$ 1.390} & \textbf{15.642 $\pm$ 1.475} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/b/table-combined-95-gamma-lambda-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (b) CLEAR calibration parameters $\lambda$ and $\gamma_1$ for 95\% prediction intervals across 10 seeds. Using all available variables. Showing median [min:max] values.}
\label{tab:combined_gamma_lambda_95_final_conformalized_variant_b}
\small
\begin{tabular}{lccc}
\toprule
Dataset & $\lambda$ & $\gamma_1$ \\
\midrule
ailerons & 0.76 [0.50:1.70] & 1.02 [0.76:1.11] \\
airfoil & 0.38 [0.14:1.14] & 1.64 [0.84:2.66] \\
allstate & 0.35 [0.00:2.75] & 1.55 [0.60:1.91] \\
ca\textunderscore housing & 0.53 [0.39:0.67] & 1.14 [1.04:1.29] \\
computer & 0.57 [0.24:0.76] & 1.15 [1.05:1.37] \\
concrete & 2.55 [0.11:100.00] & 0.60 [0.02:3.01] \\
elevator & 0.59 [0.39:0.93] & 1.10 [0.90:1.23] \\
energy\textunderscore efficiency & 0.08 [0.00:100.00] & 2.15 [0.02:3.20] \\
insurance & 0.23 [0.08:0.70] & 1.96 [1.60:2.97] \\
kin8nm & 0.99 [0.76:1.89] & 1.08 [0.72:1.28] \\
miami\textunderscore housing & 0.38 [0.16:3.70] & 1.28 [0.37:1.64] \\
naval\textunderscore propulsion & 0.01 [0.00:0.04] & 2.03 [1.56:2.32] \\
parkinsons & 0.64 [0.49:1.10] & 1.16 [0.93:1.32] \\
powerplant & 1.87 [0.95:3.78] & 0.73 [0.43:0.93] \\
qsar & 0.74 [0.46:1.83] & 1.17 [0.78:1.47] \\
sulfur & 0.47 [0.01:4.32] & 1.31 [0.53:1.78] \\
superconductor & 0.83 [0.56:1.16] & 0.89 [0.80:1.03] \\
\bottomrule
\end{tabular}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/b/table-combined-95-mpiw-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (b) MPIW at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_mpiw_95_final_conformalized_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR \\
\midrule
ailerons & \textbf{5.8e-04 $\pm$ 1.3e-05} & 6.5e-04 $\pm$ 2.3e-05 & 5.8e-04 $\pm$ 1.7e-05 & \underline{5.8e-04 $\pm$ 9.3e-06} \\
airfoil & \underline{7.346 $\pm$ 0.715} & 7.438 $\pm$ 0.896 & 7.798 $\pm$ 1.239 & \textbf{7.101 $\pm$ 0.481} \\
allstate & \underline{6.3e+03 $\pm$ 3.3e+02} & 6.4e+03 $\pm$ 5.3e+02 & 6.4e+03 $\pm$ 4.5e+02 & \textbf{6.3e+03 $\pm$ 2.4e+02} \\
ca\textunderscore housing & \underline{1.6e+05 $\pm$ 3.8e+03} & 1.7e+05 $\pm$ 6.5e+03 & 1.7e+05 $\pm$ 4.7e+03 & \textbf{1.6e+05 $\pm$ 4.5e+03} \\
computer & \textbf{9.803 $\pm$ 0.620} & \textcolor{red}{14.011 $\pm$ 0.948} & 10.310 $\pm$ 0.502 & \underline{9.833 $\pm$ 0.565} \\
concrete & 20.302 $\pm$ 1.776 & \textbf{18.730 $\pm$ 3.172} & 20.552 $\pm$ 3.407 & \underline{18.917 $\pm$ 1.985} \\
elevator & \textbf{8.5e-03 $\pm$ 2.2e-04} & \textcolor{red}{0.012 $\pm$ 0.000} & 9.0e-03 $\pm$ 3.5e-04 & \underline{8.5e-03 $\pm$ 1.2e-04} \\
energy\textunderscore efficiency & 1.940 $\pm$ 0.324 & 2.117 $\pm$ 0.326 & \underline{1.922 $\pm$ 0.348} & \textbf{1.713 $\pm$ 0.193} \\
insurance & \underline{2.0e+04 $\pm$ 2.5e+03} & \textcolor{red}{2.6e+04 $\pm$ 1.7e+04} & 2.4e+04 $\pm$ 6.7e+03 & \textbf{1.9e+04 $\pm$ 2.6e+03} \\
kin8nm & \underline{0.500 $\pm$ 0.009} & 0.515 $\pm$ 0.011 & 0.510 $\pm$ 0.010 & \textbf{0.496 $\pm$ 0.007} \\
miami\textunderscore housing & \underline{2.2e+05 $\pm$ 7.5e+03} & 2.5e+05 $\pm$ 5.8e+03 & 2.2e+05 $\pm$ 1.3e+04 & \textbf{2.2e+05 $\pm$ 4.9e+03} \\
naval\textunderscore propulsion & \underline{3.3e-03 $\pm$ 1.6e-04} & \textcolor{red}{0.014 $\pm$ 0.001} & 3.4e-03 $\pm$ 1.8e-04 & \textbf{3.3e-03 $\pm$ 1.3e-04} \\
parkinsons & \textbf{13.405 $\pm$ 0.650} & 15.607 $\pm$ 0.785 & 14.653 $\pm$ 0.593 & \underline{13.507 $\pm$ 0.448} \\
powerplant & \underline{12.309 $\pm$ 0.560} & 12.897 $\pm$ 0.433 & 13.152 $\pm$ 0.343 & \textbf{12.232 $\pm$ 0.274} \\
qsar & \underline{3.152 $\pm$ 0.137} & 3.359 $\pm$ 0.157 & 3.294 $\pm$ 0.114 & \textbf{3.114 $\pm$ 0.100} \\
sulfur & 0.101 $\pm$ 0.005 & 0.118 $\pm$ 0.007 & \textbf{0.097 $\pm$ 0.005} & \underline{0.098 $\pm$ 0.003} \\
superconductor & \underline{31.752 $\pm$ 0.892} & 34.655 $\pm$ 1.027 & 32.766 $\pm$ 0.869 & \textbf{31.534 $\pm$ 0.797} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/b/table-uncertainty-metrics-95_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (b) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_conformalized_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.42 [0.28:0.94] \\
airfoil & 4.24 [2.33:6.69] & 2.81 [1.60:4.77] & 0.70 [0.24:2.04] \\
allstate & 5477.71 [2089.01:6430.35] & 1194.83 [0.00:3531.52] & 0.24 [0.00:1.69] \\
ca\textunderscore housing & 124233.23 [116128.73:140499.66] & 36688.78 [30210.52:42274.41] & 0.29 [0.22:0.36] \\
computer & 5.63 [5.02:6.67] & 4.34 [2.37:5.61] & 0.82 [0.35:1.08] \\
concrete & 3.40 [0.08:17.11] & 16.37 [3.89:18.84] & 5.14 [0.23:217.70] \\
elevator & 0.01 [0.00:0.01] & 0.00 [0.00:0.00] & 0.39 [0.26:0.62] \\
energy\textunderscore efficiency & 1.41 [0.01:1.78] & 0.32 [0.00:2.68] & 0.21 [0.00:256.94] \\
insurance & 15957.40 [13981.72:23994.95] & 2794.74 [1360.44:8787.67] & 0.17 [0.06:0.55] \\
kin8nm & 0.23 [0.16:0.27] & 0.27 [0.23:0.35] & 1.16 [0.88:2.17] \\
miami\textunderscore housing & 147841.18 [42132.61:190207.05] & 66143.03 [37463.58:185821.66] & 0.44 [0.20:4.41] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.10 [0.00:0.39] \\
parkinsons & 7.61 [5.95:8.95] & 5.24 [4.50:7.23] & 0.68 [0.50:1.14] \\
powerplant & 5.84 [3.51:7.53] & 6.89 [4.53:8.31] & 1.17 [0.60:2.37] \\
qsar & 1.88 [1.29:2.35] & 1.26 [0.93:2.03] & 0.67 [0.41:1.58] \\
sulfur & 0.08 [0.03:0.10] & 0.02 [0.00:0.07] & 0.25 [0.01:2.25] \\
superconductor & 22.24 [20.05:25.61] & 9.54 [7.26:12.22] & 0.42 [0.28:0.60] \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/c/table-combined-95-crps-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (c) CRPS at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result. $+\infty$ indicates UACQR-P produced infinitely wide intervals; superscripts show affected/total seeds, subscripts the finite-seed mean.}
\label{tab:combined_crps_95_final_conformalized_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR & UACQR-P & UACQR-S \\
\midrule
ailerons & 9.2e-05 $\pm$ 1.3e-06 & 9.7e-05 $\pm$ 1.9e-06 & \underline{9.2e-05 $\pm$ 1.2e-06} & 9.2e-05 $\pm$ 1.8e-06 & \textbf{8.9e-05 $\pm$ 1.3e-06} & 9.4e-05 $\pm$ 1.4e-06 \\
airfoil & 1.011 $\pm$ 0.077 & 1.057 $\pm$ 0.085 & \underline{0.999 $\pm$ 0.103} & \textbf{0.997 $\pm$ 0.080} & \textcolor{red}{1.836 $\pm$ 0.107} & \textcolor{red}{1.920 $\pm$ 0.095} \\
allstate & 1.1e+03 $\pm$ 77.998 & \textbf{1.1e+03 $\pm$ 35.601} & \underline{1.1e+03 $\pm$ 51.011} & 1.1e+03 $\pm$ 64.894 & 1.2e+03 $\pm$ 46.822 & 1.3e+03 $\pm$ 58.594 \\
ca\textunderscore housing & \underline{2.3e+04 $\pm$ 3.0e+02} & 2.4e+04 $\pm$ 4.0e+02 & 2.4e+04 $\pm$ 2.9e+02 & \textbf{2.3e+04 $\pm$ 3.3e+02} & 2.9e+04 $\pm$ 4.7e+02 & \textcolor{red}{3.2e+04 $\pm$ 4.3e+02} \\
computer & \textbf{1.202 $\pm$ 0.040} & 1.226 $\pm$ 0.050 & 1.240 $\pm$ 0.028 & \underline{1.218 $\pm$ 0.061} & 1.373 $\pm$ 0.033 & 1.517 $\pm$ 0.029 \\
concrete & 3.321 $\pm$ 0.317 & 3.282 $\pm$ 0.290 & \textbf{2.850 $\pm$ 0.249} & \underline{3.227 $\pm$ 0.280} & \textcolor{red}{4.040 $\pm$ 0.189} & \textcolor{red}{4.232 $\pm$ 0.159} \\
elevator & \textbf{1.2e-03 $\pm$ 7.7e-06} & 1.3e-03 $\pm$ 2.1e-05 & 1.2e-03 $\pm$ 1.7e-05 & \underline{1.2e-03 $\pm$ 1.1e-05} & \textcolor{red}{1.7e-03 $\pm$ 2.6e-05} & \textcolor{red}{1.9e-03 $\pm$ 2.3e-05} \\
energy\textunderscore efficiency & 0.277 $\pm$ 0.032 & 0.275 $\pm$ 0.037 & \textbf{0.246 $\pm$ 0.030} & \underline{0.249 $\pm$ 0.030} & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny 0.884}}$ & \textcolor{red}{0.926 $\pm$ 0.070} \\
insurance & 4.1e+03 $\pm$ 7.2e+02 & \textbf{3.3e+03 $\pm$ 6.7e+02} & 4.4e+03 $\pm$ 9.4e+02 & \underline{3.8e+03 $\pm$ 6.1e+02} & 4.0e+03 $\pm$ 3.0e+02 & 4.2e+03 $\pm$ 3.0e+02 \\
kin8nm & 0.067 $\pm$ 0.002 & \underline{0.067 $\pm$ 0.001} & 0.067 $\pm$ 0.002 & \textbf{0.067 $\pm$ 0.001} & \textcolor{red}{0.097 $\pm$ 0.002} & \textcolor{red}{0.099 $\pm$ 0.002} \\
miami\textunderscore housing & \underline{3.4e+04 $\pm$ 1.0e+03} & 3.5e+04 $\pm$ 1.8e+03 & 4.1e+04 $\pm$ 3.1e+03 & \textbf{3.4e+04 $\pm$ 8.1e+02} & 4.0e+04 $\pm$ 8.8e+02 & 4.4e+04 $\pm$ 9.0e+02 \\
naval\textunderscore propulsion & \underline{4.2e-04 $\pm$ 7.0e-06} & 4.3e-04 $\pm$ 9.4e-06 & 4.3e-04 $\pm$ 9.7e-06 & \textbf{4.2e-04 $\pm$ 7.7e-06} & \textcolor{red}{5.9e-04 $\pm$ 1.7e-05} & \textcolor{red}{7.7e-04 $\pm$ 1.7e-05} \\
parkinsons & \textbf{1.863 $\pm$ 0.046} & 1.948 $\pm$ 0.044 & 1.876 $\pm$ 0.026 & \underline{1.866 $\pm$ 0.042} & 2.415 $\pm$ 0.140 & \textcolor{red}{2.737 $\pm$ 0.144} \\
powerplant & 1.768 $\pm$ 0.035 & 1.897 $\pm$ 0.042 & \textbf{1.716 $\pm$ 0.033} & \underline{1.763 $\pm$ 0.028} & 2.172 $\pm$ 0.044 & 2.270 $\pm$ 0.040 \\
qsar & 0.458 $\pm$ 0.015 & 0.521 $\pm$ 0.016 & \textbf{0.450 $\pm$ 0.011} & \underline{0.454 $\pm$ 0.013} & 0.581 $\pm$ 0.009 & \textcolor{red}{0.614 $\pm$ 0.012} \\
sulfur & 0.017 $\pm$ 0.001 & 0.018 $\pm$ 0.000 & \textbf{0.016 $\pm$ 0.001} & \underline{0.017 $\pm$ 0.001} & 0.019 $\pm$ 0.001 & \textcolor{red}{0.022 $\pm$ 0.001} \\
superconductor & \underline{4.628 $\pm$ 0.107} & 5.193 $\pm$ 0.150 & 4.695 $\pm$ 0.130 & \textbf{4.597 $\pm$ 0.132} & 5.455 $\pm$ 0.145 & 5.722 $\pm$ 0.129 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/c/table-combined-95-expectileloss-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (c) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result. $+\infty$ indicates UACQR-P produced infinitely wide intervals; superscripts show affected/total seeds, subscripts the finite-seed mean.}
\label{tab:combined_expectileloss_95_final_conformalized_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR & UACQR-P & UACQR-S \\
\midrule
ailerons & 3.7e-09 $\pm$ 2.0e-10 & \textcolor{red}{5.3e-09 $\pm$ 4.8e-10} & \underline{3.6e-09 $\pm$ 1.4e-10} & 3.7e-09 $\pm$ 1.5e-10 & \textbf{3.4e-09 $\pm$ 1.3e-10} & 4.1e-09 $\pm$ 1.2e-10 \\
airfoil & \underline{0.522 $\pm$ 0.108} & 0.547 $\pm$ 0.131 & 0.582 $\pm$ 0.172 & \textbf{0.485 $\pm$ 0.110} & \textcolor{red}{1.418 $\pm$ 0.177} & \textcolor{red}{1.604 $\pm$ 0.151} \\
allstate & \underline{6.2e+05 $\pm$ 4.3e+04} & 7.3e+05 $\pm$ 9.0e+04 & 6.4e+05 $\pm$ 1.4e+05 & \textbf{6.0e+05 $\pm$ 4.2e+04} & 6.5e+05 $\pm$ 8.7e+04 & 7.4e+05 $\pm$ 7.3e+04 \\
ca\textunderscore housing & \underline{2.9e+08 $\pm$ 1.3e+07} & 3.2e+08 $\pm$ 1.7e+07 & 3.3e+08 $\pm$ 1.1e+07 & \textbf{2.9e+08 $\pm$ 1.3e+07} & \textcolor{red}{3.9e+08 $\pm$ 1.0e+07} & \textcolor{red}{4.5e+08 $\pm$ 8.1e+06} \\
computer & \textcolor{red}{1.281 $\pm$ 0.687} & \textcolor{red}{1.364 $\pm$ 0.657} & \textcolor{red}{1.409 $\pm$ 0.800} & \textcolor{red}{1.177 $\pm$ 0.662} & \textbf{0.858 $\pm$ 0.062} & \underline{1.103 $\pm$ 0.063} \\
concrete & 5.110 $\pm$ 1.087 & \textbf{4.722 $\pm$ 0.971} & 4.912 $\pm$ 1.358 & \underline{4.804 $\pm$ 0.906} & \textcolor{red}{6.972 $\pm$ 0.622} & \textcolor{red}{7.969 $\pm$ 0.610} \\
elevator & \textbf{6.5e-07 $\pm$ 1.5e-08} & \textcolor{red}{9.4e-07 $\pm$ 4.1e-08} & 7.5e-07 $\pm$ 4.4e-08 & \underline{6.5e-07 $\pm$ 1.4e-08} & \textcolor{red}{1.3e-06 $\pm$ 4.7e-08} & \textcolor{red}{1.7e-06 $\pm$ 5.5e-08} \\
energy\textunderscore efficiency & 0.052 $\pm$ 0.017 & \textcolor{red}{0.054 $\pm$ 0.025} & \underline{0.049 $\pm$ 0.035} & \textbf{0.040 $\pm$ 0.019} & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny 0.372}}$ & \textcolor{red}{0.393 $\pm$ 0.031} \\
insurance & \textcolor{red}{6.5e+06 $\pm$ 2.5e+06} & \textcolor{red}{6.5e+06 $\pm$ 2.6e+06} & \textcolor{red}{6.1e+06 $\pm$ 1.1e+06} & \textcolor{red}{6.8e+06 $\pm$ 2.9e+06} & \textbf{4.5e+06 $\pm$ 6.0e+05} & \underline{4.9e+06 $\pm$ 7.0e+05} \\
kin8nm & \underline{1.8e-03 $\pm$ 9.1e-05} & 1.8e-03 $\pm$ 7.4e-05 & 1.8e-03 $\pm$ 1.0e-04 & \textbf{1.7e-03 $\pm$ 7.3e-05} & \textcolor{red}{3.3e-03 $\pm$ 1.2e-04} & \textcolor{red}{3.4e-03 $\pm$ 9.2e-05} \\
miami\textunderscore housing & \underline{1.1e+09 $\pm$ 1.3e+08} & 1.3e+09 $\pm$ 1.9e+08 & \textcolor{red}{1.9e+09 $\pm$ 3.5e+08} & \textbf{1.1e+09 $\pm$ 6.9e+07} & \textcolor{red}{1.5e+09 $\pm$ 8.3e+07} & \textcolor{red}{1.8e+09 $\pm$ 8.6e+07} \\
naval\textunderscore propulsion & \textbf{8.1e-08 $\pm$ 2.5e-09} & 1.0e-07 $\pm$ 7.7e-09 & 8.5e-08 $\pm$ 4.9e-09 & \underline{8.1e-08 $\pm$ 3.2e-09} & \textcolor{red}{5.8e-07 $\pm$ 1.6e-07} & \textcolor{red}{7.4e-07 $\pm$ 3.9e-08} \\
parkinsons & \underline{1.402 $\pm$ 0.091} & 1.541 $\pm$ 0.088 & 1.582 $\pm$ 0.093 & \textbf{1.400 $\pm$ 0.045} & \textcolor{red}{1.969 $\pm$ 0.248} & \textcolor{red}{2.574 $\pm$ 0.276} \\
powerplant & 1.784 $\pm$ 0.378 & 1.992 $\pm$ 0.331 & \underline{1.776 $\pm$ 0.372} & \textbf{1.771 $\pm$ 0.379} & 2.214 $\pm$ 0.345 & \textcolor{red}{2.418 $\pm$ 0.291} \\
qsar & 0.107 $\pm$ 0.026 & \textcolor{red}{0.141 $\pm$ 0.021} & \textbf{0.102 $\pm$ 0.028} & \underline{0.103 $\pm$ 0.027} & 0.128 $\pm$ 0.026 & \textcolor{red}{0.147 $\pm$ 0.020} \\
sulfur & \underline{2.3e-04 $\pm$ 1.8e-05} & 2.8e-04 $\pm$ 2.2e-05 & \textcolor{red}{3.5e-04 $\pm$ 6.4e-05} & \textbf{2.2e-04 $\pm$ 1.5e-05} & 2.9e-04 $\pm$ 6.2e-05 & \textcolor{red}{3.4e-04 $\pm$ 6.5e-05} \\
superconductor & 13.409 $\pm$ 1.146 & \textcolor{red}{19.306 $\pm$ 1.443} & \underline{13.211 $\pm$ 1.709} & \textbf{13.197 $\pm$ 1.496} & 16.194 $\pm$ 1.575 & 17.417 $\pm$ 1.301 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/c/table-combined-95-mpiw-final_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (c) MPIW at 95\% prediction intervals, aggregated across 10 seeds. Methods with suffix `-c' denote conformalized variants obtained using the validation set divided into two parts, one for validation and one for calibration.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result. $+\infty$ indicates UACQR-P produced infinitely wide intervals; superscripts show affected/total seeds, subscripts the finite-seed mean.}
\label{tab:combined_mpiw_95_final_conformalized_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Dataset & CLEAR-c & PCS-EPISTEMIC-c & ALEATORIC-R-c & CLEAR & UACQR-P & UACQR-S \\
\midrule
ailerons & 6.2e-04 $\pm$ 2.0e-05 & \textcolor{red}{7.2e-04 $\pm$ 3.5e-05} & \underline{6.0e-04 $\pm$ 1.5e-05} & 6.2e-04 $\pm$ 1.1e-05 & \textbf{5.3e-04 $\pm$ 9.2e-06} & 6.2e-04 $\pm$ 8.3e-06 \\
airfoil & \underline{7.177 $\pm$ 0.725} & 7.260 $\pm$ 0.891 & 7.897 $\pm$ 1.431 & \textbf{6.822 $\pm$ 0.602} & \textcolor{red}{12.565 $\pm$ 0.949} & \textcolor{red}{13.489 $\pm$ 0.845} \\
allstate & \underline{6.9e+03 $\pm$ 4.7e+02} & 7.1e+03 $\pm$ 3.7e+02 & 6.9e+03 $\pm$ 7.9e+02 & \textbf{6.8e+03 $\pm$ 2.9e+02} & 7.0e+03 $\pm$ 2.3e+02 & 7.5e+03 $\pm$ 2.8e+02 \\
ca\textunderscore housing & \underline{1.5e+05 $\pm$ 4.9e+03} & 1.6e+05 $\pm$ 7.1e+03 & 1.7e+05 $\pm$ 5.4e+03 & \textbf{1.5e+05 $\pm$ 5.3e+03} & 1.8e+05 $\pm$ 2.8e+03 & 2.0e+05 $\pm$ 1.8e+03 \\
computer & \textbf{7.857 $\pm$ 0.310} & 8.185 $\pm$ 0.322 & 8.725 $\pm$ 0.352 & \underline{7.954 $\pm$ 0.388} & 8.238 $\pm$ 0.324 & 10.080 $\pm$ 0.120 \\
concrete & 21.993 $\pm$ 2.873 & \textbf{20.734 $\pm$ 2.472} & 21.780 $\pm$ 2.774 & \underline{21.075 $\pm$ 2.217} & \textcolor{red}{28.647 $\pm$ 1.522} & \textcolor{red}{30.727 $\pm$ 1.645} \\
elevator & \textbf{7.8e-03 $\pm$ 2.2e-04} & 9.5e-03 $\pm$ 2.3e-04 & 8.4e-03 $\pm$ 2.8e-04 & \underline{7.9e-03 $\pm$ 1.3e-04} & 9.8e-03 $\pm$ 2.2e-04 & \textcolor{red}{0.012 $\pm$ 0.000} \\
energy\textunderscore efficiency & 1.905 $\pm$ 0.269 & \underline{1.581 $\pm$ 0.284} & 1.929 $\pm$ 0.252 & \textbf{1.577 $\pm$ 0.261} & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny 5.615}}$ & \textcolor{red}{5.715 $\pm$ 0.206} \\
insurance & \textcolor{red}{2.3e+04 $\pm$ 5.0e+03} & 2.2e+04 $\pm$ 7.8e+03 & \textcolor{red}{2.5e+04 $\pm$ 5.3e+03} & 2.3e+04 $\pm$ 6.2e+03 & \textbf{1.7e+04 $\pm$ 1.9e+03} & \underline{1.8e+04 $\pm$ 1.5e+03} \\
kin8nm & 0.453 $\pm$ 0.017 & \underline{0.451 $\pm$ 0.011} & 0.452 $\pm$ 0.017 & \textbf{0.448 $\pm$ 0.012} & \textcolor{red}{0.612 $\pm$ 0.015} & \textcolor{red}{0.624 $\pm$ 0.010} \\
miami\textunderscore housing & \underline{2.3e+05 $\pm$ 7.6e+03} & 2.5e+05 $\pm$ 1.4e+04 & 2.9e+05 $\pm$ 4.7e+04 & \textbf{2.3e+05 $\pm$ 3.6e+03} & 2.7e+05 $\pm$ 6.3e+03 & 2.9e+05 $\pm$ 6.7e+03 \\
naval\textunderscore propulsion & \underline{2.8e-03 $\pm$ 6.2e-05} & 3.0e-03 $\pm$ 1.2e-04 & 2.9e-03 $\pm$ 8.5e-05 & \textbf{2.8e-03 $\pm$ 5.6e-05} & 3.0e-03 $\pm$ 7.6e-05 & \textcolor{red}{6.2e-03 $\pm$ 1.4e-04} \\
parkinsons & \textbf{11.986 $\pm$ 0.700} & 12.564 $\pm$ 0.455 & 13.500 $\pm$ 0.725 & \underline{11.990 $\pm$ 0.335} & 12.991 $\pm$ 0.962 & 15.093 $\pm$ 0.926 \\
powerplant & \underline{11.348 $\pm$ 0.593} & 12.228 $\pm$ 0.285 & 11.666 $\pm$ 0.409 & \textbf{11.293 $\pm$ 0.302} & 13.913 $\pm$ 0.364 & 14.618 $\pm$ 0.357 \\
qsar & 3.005 $\pm$ 0.107 & 3.392 $\pm$ 0.205 & \underline{2.978 $\pm$ 0.110} & \textbf{2.931 $\pm$ 0.130} & 3.491 $\pm$ 0.102 & 3.811 $\pm$ 0.082 \\
sulfur & 0.102 $\pm$ 0.007 & 0.115 $\pm$ 0.004 & \textbf{0.098 $\pm$ 0.010} & \underline{0.101 $\pm$ 0.004} & 0.105 $\pm$ 0.005 & 0.115 $\pm$ 0.005 \\
superconductor & \underline{28.316 $\pm$ 0.894} & 33.797 $\pm$ 1.156 & 30.043 $\pm$ 1.962 & \textbf{28.088 $\pm$ 0.812} & 31.606 $\pm$ 0.708 & 33.676 $\pm$ 0.592 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/c/table-uncertainty-metrics-95_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Conformalized Variant (c) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_conformalized_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.31 [0.08:0.56] \\
airfoil & 0.88 [0.01:3.81] & 6.22 [3.29:7.40] & 8.02 [0.88:701.30] \\
allstate & 5640.21 [33.18:7348.98] & 1399.92 [0.00:6669.67] & 0.25 [0.00:185.01] \\
ca\textunderscore housing & 52486.01 [10675.87:73733.36] & 96584.89 [77553.77:141987.21] & 1.84 [1.05:13.30] \\
computer & 1.23 [0.38:2.00] & 6.69 [5.53:7.76] & 5.64 [2.83:20.44] \\
concrete & 1.43 [0.02:3.70] & 18.94 [14.65:25.73] & 13.75 [3.96:1325.80] \\
elevator & 0.00 [0.00:0.01] & 0.00 [0.00:0.00] & 0.84 [0.49:1.41] \\
energy\textunderscore efficiency & 0.47 [0.00:1.34] & 1.31 [0.43:2.30] & 3.20 [0.32:1450.65] \\
insurance & 6114.71 [16.49:14708.51] & 15632.81 [9873.62:35076.03] & 2.49 [0.74:1640.72] \\
kin8nm & 0.27 [0.23:0.38] & 0.18 [0.05:0.23] & 0.68 [0.12:1.02] \\
miami\textunderscore housing & 25504.25 [1244.93:163459.56] & 199473.12 [72446.41:223498.23] & 8.01 [0.44:179.53] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 1.52 [1.05:2.40] \\
parkinsons & 2.87 [0.26:4.88] & 9.03 [7.09:11.39] & 3.31 [1.62:43.94] \\
powerplant & 5.33 [2.40:6.66] & 5.94 [4.04:9.15] & 1.10 [0.64:3.82] \\
qsar & 2.17 [0.68:2.42] & 0.86 [0.47:2.33] & 0.38 [0.19:3.42] \\
sulfur & 0.02 [0.00:0.04] & 0.08 [0.05:0.10] & 2.95 [1.25:131.28] \\
superconductor & 21.97 [12.60:26.52] & 6.50 [2.20:15.67] & 0.30 [0.08:1.24] \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/conformalized/table-clear-vs-uacqr-improvement-95_conformalized.tex <==
\begin{table}[!htbp]
\centering
\caption{Improvement (\%) of conformalized CLEAR-c variant (c) over UACQR-S and UACQR-P at 95\% coverage across 17 datasets. \textbf{Bold values with +} indicate CLEAR-c outperforms the baseline. $+\infty^{1/10}_{v}$ denotes that UACQR-P produced infinitely wide intervals for $1$ out of the $10$ seeds, and the mean improvement on the remaining $9$ seeds was $v$.}
\label{tab:clear_vs_uacqr_detailed_conformalized}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Dataset & \multicolumn{3}{c}{UACQR-S} & \multicolumn{3}{c}{UACQR-P} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & NCIW & AISL & Width & NCIW & AISL & Width \\
\midrule
ailerons & -0.9\% & \textbf{+3.3\%} & -0.2\% & -8.7\% & \textbf{+2.8\%} & -18.0\% \\
airfoil & \textbf{+39.9\%} & \textbf{+43.2\%} & \textbf{+46.8\%} & \textbf{+40.3\%} & \textbf{+41.9\%} & \textbf{+42.9\%} \\
allstate & \textbf{+8.0\%} & -0.2\% & \textbf{+8.0\%} & \textbf{+1.7\%} & -4.7\% & \textbf{+1.0\%} \\
ca\_housing & \textbf{+23.1\%} & \textbf{+8.7\%} & \textbf{+21.8\%} & \textbf{+14.7\%} & \textbf{+5.6\%} & \textbf{+13.2\%} \\
computer & \textbf{+21.9\%} & \textbf{+9.0\%} & \textbf{+22.1\%} & \textbf{+8.4\%} & \textbf{+6.0\%} & \textbf{+4.6\%} \\
concrete & \textbf{+22.4\%} & \textbf{+19.6\%} & \textbf{+28.4\%} & \textbf{+23.1\%} & \textbf{+16.7\%} & \textbf{+23.2\%} \\
elevator & \textbf{+36.5\%} & \textbf{+28.8\%} & \textbf{+36.6\%} & \textbf{+24.5\%} & \textbf{+27.2\%} & \textbf{+19.9\%} \\
energy\_efficiency & \textbf{+68.4\%} & \textbf{+60.5\%} & \textbf{+66.7\%} & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny \textbf{+69.4\%}}}$ & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny \textbf{+61.0\%}}}$ & $+\infty^{\text{\tiny 1/10}}_{\text{\tiny \textbf{+66.8\%}}}$ \\
insurance & -19.0\% & -15.7\% & -32.9\% & -22.2\% & -19.6\% & -36.4\% \\
kin8nm & \textbf{+27.3\%} & \textbf{+26.5\%} & \textbf{+27.5\%} & \textbf{+26.0\%} & \textbf{+23.9\%} & \textbf{+26.1\%} \\
miami\_housing & \textbf{+20.7\%} & \textbf{+17.9\%} & \textbf{+22.8\%} & \textbf{+14.6\%} & \textbf{+13.1\%} & \textbf{+15.2\%} \\
naval\_propulsion & \textbf{+55.9\%} & \textbf{+51.8\%} & \textbf{+55.3\%} & \textbf{+7.4\%} & \textbf{+59.1\%} & \textbf{+6.2\%} \\
parkinsons & \textbf{+20.6\%} & \textbf{+4.6\%} & \textbf{+20.6\%} & \textbf{+8.9\%} & -5.1\% & \textbf{+7.7\%} \\
powerplant & \textbf{+19.2\%} & \textbf{+13.2\%} & \textbf{+22.4\%} & \textbf{+14.9\%} & \textbf{+9.8\%} & \textbf{+18.4\%} \\
qsar & \textbf{+21.0\%} & \textbf{+9.7\%} & \textbf{+21.2\%} & \textbf{+14.5\%} & \textbf{+4.8\%} & \textbf{+13.9\%} \\
sulfur & \textbf{+12.2\%} & \textbf{+9.6\%} & \textbf{+11.1\%} & \textbf{+3.6\%} & \textbf{+5.3\%} & \textbf{+2.4\%} \\
superconductor & \textbf{+16.6\%} & \textbf{+6.5\%} & \textbf{+15.9\%} & \textbf{+11.4\%} & \textbf{+3.9\%} & \textbf{+10.4\%} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tex_tbls/pcs_cqr/standard/a/table-combined-95-crps-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (a) CRPS at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_crps_95_final_standard_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & \underline{8.6e-05 $\pm$ 7.9e-07} & 9.6e-05 $\pm$ 1.4e-06 & 8.7e-05 $\pm$ 9.6e-07 & 8.9e-05 $\pm$ 7.8e-07 & 9.1e-05 $\pm$ 1.2e-06 & 8.6e-05 $\pm$ 8.5e-07 & \textbf{8.6e-05 $\pm$ 8.2e-07} \\
airfoil & 1.083 $\pm$ 0.062 & \textcolor{red}{2.192 $\pm$ 0.084} & 1.075 $\pm$ 0.068 & 1.109 $\pm$ 0.061 & 1.135 $\pm$ 0.080 & \underline{1.072 $\pm$ 0.058} & \textbf{1.072 $\pm$ 0.058} \\
allstate & 1.1e+03 $\pm$ 43.869 & 1.2e+03 $\pm$ 34.114 & 1.0e+03 $\pm$ 29.034 & \textbf{9.9e+02 $\pm$ 46.205} & 1.1e+03 $\pm$ 44.717 & \underline{1.0e+03 $\pm$ 29.594} & 1.0e+03 $\pm$ 30.168 \\
ca\textunderscore housing & 2.6e+04 $\pm$ 4.2e+02 & \textcolor{red}{8.3e+04 $\pm$ 6.9e+02} & 2.6e+04 $\pm$ 3.1e+02 & \underline{2.5e+04 $\pm$ 3.9e+02} & 2.8e+04 $\pm$ 3.2e+02 & 2.5e+04 $\pm$ 3.3e+02 & \textbf{2.5e+04 $\pm$ 3.3e+02} \\
computer & \underline{1.370 $\pm$ 0.123} & 1.471 $\pm$ 0.040 & 1.378 $\pm$ 0.116 & \textcolor{red}{2.2e+02 $\pm$ 1.4e+02} & 1.520 $\pm$ 0.052 & \textbf{1.367 $\pm$ 0.136} & 1.371 $\pm$ 0.130 \\
concrete & 2.927 $\pm$ 0.259 & \textcolor{red}{6.393 $\pm$ 0.361} & \underline{2.844 $\pm$ 0.256} & 2.974 $\pm$ 0.228 & \textbf{2.827 $\pm$ 0.257} & 2.918 $\pm$ 0.236 & 2.922 $\pm$ 0.235 \\
elevator & 1.5e-03 $\pm$ 1.3e-05 & \underline{1.4e-03 $\pm$ 8.5e-06} & 1.4e-03 $\pm$ 1.0e-05 & 1.5e-03 $\pm$ 1.9e-05 & \textbf{1.3e-03 $\pm$ 1.2e-05} & 1.4e-03 $\pm$ 7.8e-06 & 1.5e-03 $\pm$ 1.4e-05 \\
energy\textunderscore efficiency & \underline{0.274 $\pm$ 0.029} & \textcolor{red}{1.842 $\pm$ 0.138} & \textbf{0.262 $\pm$ 0.022} & \textcolor{red}{0.371 $\pm$ 0.030} & 0.293 $\pm$ 0.031 & 0.304 $\pm$ 0.025 & 0.313 $\pm$ 0.023 \\
insurance & \textcolor{red}{4.7e+03 $\pm$ 3.4e+02} & \underline{3.6e+03 $\pm$ 1.6e+02} & \textcolor{red}{4.0e+03 $\pm$ 3.6e+02} & \textcolor{red}{4.4e+03 $\pm$ 9.5e+02} & \textbf{3.0e+03 $\pm$ 3.3e+02} & \textcolor{red}{4.2e+03 $\pm$ 1.9e+02} & \textcolor{red}{4.2e+03 $\pm$ 4.0e+02} \\
kin8nm & \underline{0.076 $\pm$ 0.001} & \textcolor{red}{0.111 $\pm$ 0.001} & 0.077 $\pm$ 0.001 & 0.077 $\pm$ 0.001 & 0.078 $\pm$ 0.001 & \textbf{0.076 $\pm$ 0.001} & 0.076 $\pm$ 0.001 \\
miami\textunderscore housing & 3.4e+04 $\pm$ 9.5e+02 & \textcolor{red}{4.6e+04 $\pm$ 1.3e+03} & 3.6e+04 $\pm$ 1.1e+03 & 3.6e+04 $\pm$ 9.2e+02 & 4.5e+04 $\pm$ 1.2e+03 & \textbf{3.4e+04 $\pm$ 9.5e+02} & \underline{3.4e+04 $\pm$ 9.5e+02} \\
naval\textunderscore propulsion & 1.8e-04 $\pm$ 2.0e-06 & 1.8e-04 $\pm$ 2.1e-06 & \underline{1.8e-04 $\pm$ 2.1e-06} & 1.9e-04 $\pm$ 2.0e-06 & \textbf{1.8e-04 $\pm$ 2.0e-06} & 1.8e-04 $\pm$ 2.0e-06 & 1.8e-04 $\pm$ 2.1e-06 \\
parkinsons & 1.794 $\pm$ 0.072 & \textcolor{red}{2.745 $\pm$ 0.099} & 1.760 $\pm$ 0.036 & \textcolor{red}{2.535 $\pm$ 0.191} & 1.931 $\pm$ 0.048 & \textbf{1.737 $\pm$ 0.043} & \underline{1.758 $\pm$ 0.049} \\
powerplant & \underline{1.938 $\pm$ 0.034} & 2.288 $\pm$ 0.032 & 1.979 $\pm$ 0.030 & 1.938 $\pm$ 0.033 & \textbf{1.918 $\pm$ 0.024} & 1.970 $\pm$ 0.031 & 1.962 $\pm$ 0.033 \\
qsar & 0.486 $\pm$ 0.008 & \textcolor{red}{0.717 $\pm$ 0.010} & 0.490 $\pm$ 0.010 & 0.500 $\pm$ 0.008 & 0.499 $\pm$ 0.010 & \textbf{0.485 $\pm$ 0.009} & \underline{0.485 $\pm$ 0.009} \\
sulfur & 0.017 $\pm$ 0.000 & 0.018 $\pm$ 0.001 & \textbf{0.016 $\pm$ 0.000} & 0.018 $\pm$ 0.001 & 0.018 $\pm$ 0.000 & \underline{0.016 $\pm$ 0.000} & 0.016 $\pm$ 0.000 \\
superconductor & 4.558 $\pm$ 0.097 & 5.670 $\pm$ 0.100 & 4.563 $\pm$ 0.120 & 5.486 $\pm$ 0.135 & 5.903 $\pm$ 0.130 & \underline{4.548 $\pm$ 0.104} & \textbf{4.545 $\pm$ 0.103} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/a/table-combined-95-expectileloss-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (a) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_expectileloss_95_final_standard_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & 3.3e-09 $\pm$ 1.0e-10 & 4.0e-09 $\pm$ 1.7e-10 & 3.4e-09 $\pm$ 1.6e-10 & 4.2e-09 $\pm$ 9.6e-11 & 4.1e-09 $\pm$ 2.4e-10 & \textbf{3.3e-09 $\pm$ 1.0e-10} & \underline{3.3e-09 $\pm$ 1.0e-10} \\
airfoil & 0.499 $\pm$ 0.071 & \textcolor{red}{1.507 $\pm$ 0.123} & 0.528 $\pm$ 0.111 & 0.557 $\pm$ 0.088 & \textcolor{red}{0.687 $\pm$ 0.166} & \textbf{0.491 $\pm$ 0.071} & \underline{0.492 $\pm$ 0.071} \\
allstate & 5.8e+05 $\pm$ 9.6e+04 & 6.7e+05 $\pm$ 8.2e+04 & 6.0e+05 $\pm$ 8.5e+04 & 6.1e+05 $\pm$ 9.3e+04 & \textcolor{red}{8.7e+05 $\pm$ 1.3e+05} & \textbf{5.6e+05 $\pm$ 8.0e+04} & \underline{5.6e+05 $\pm$ 8.1e+04} \\
ca\textunderscore housing & 3.2e+08 $\pm$ 6.5e+06 & \textcolor{red}{1.4e+09 $\pm$ 1.1e+07} & 3.3e+08 $\pm$ 7.0e+06 & 3.8e+08 $\pm$ 1.1e+07 & \textcolor{red}{4.6e+08 $\pm$ 9.8e+06} & \underline{3.2e+08 $\pm$ 6.9e+06} & \textbf{3.2e+08 $\pm$ 7.8e+06} \\
computer & 1.064 $\pm$ 0.636 & \underline{1.010 $\pm$ 0.051} & \textbf{0.929 $\pm$ 0.321} & \textcolor{red}{4.9e+04 $\pm$ 3.5e+04} & 1.218 $\pm$ 0.146 & \textcolor{red}{1.463 $\pm$ 1.820} & 1.081 $\pm$ 0.671 \\
concrete & 4.220 $\pm$ 0.866 & \textcolor{red}{13.021 $\pm$ 1.326} & 4.346 $\pm$ 0.984 & \textbf{4.149 $\pm$ 0.779} & 4.408 $\pm$ 1.056 & \underline{4.187 $\pm$ 0.833} & 4.221 $\pm$ 0.847 \\
elevator & 9.1e-07 $\pm$ 4.2e-08 & \textbf{8.1e-07 $\pm$ 5.5e-08} & \underline{8.6e-07 $\pm$ 4.9e-08} & \textcolor{red}{1.3e-06 $\pm$ 1.2e-07} & 9.5e-07 $\pm$ 8.5e-08 & 9.2e-07 $\pm$ 4.9e-08 & 9.5e-07 $\pm$ 3.7e-08 \\
energy\textunderscore efficiency & \underline{0.044 $\pm$ 0.012} & \textcolor{red}{0.838 $\pm$ 0.127} & \textbf{0.039 $\pm$ 0.011} & \textcolor{red}{0.079 $\pm$ 0.009} & 0.051 $\pm$ 0.013 & \textcolor{red}{0.053 $\pm$ 0.009} & \textcolor{red}{0.056 $\pm$ 0.008} \\
insurance & 5.0e+06 $\pm$ 1.1e+06 & 4.8e+06 $\pm$ 5.9e+05 & \underline{4.7e+06 $\pm$ 8.9e+05} & \textcolor{red}{1.8e+07 $\pm$ 9.9e+06} & 6.0e+06 $\pm$ 1.2e+06 & 5.3e+06 $\pm$ 1.6e+06 & \textbf{4.7e+06 $\pm$ 1.2e+06} \\
kin8nm & 2.2e-03 $\pm$ 5.4e-05 & \textcolor{red}{4.0e-03 $\pm$ 8.8e-05} & 2.3e-03 $\pm$ 8.0e-05 & 2.3e-03 $\pm$ 4.0e-05 & 2.5e-03 $\pm$ 1.0e-04 & \textbf{2.2e-03 $\pm$ 4.8e-05} & \underline{2.2e-03 $\pm$ 4.9e-05} \\
miami\textunderscore housing & \textbf{1.1e+09 $\pm$ 1.1e+08} & \textcolor{red}{1.8e+09 $\pm$ 1.7e+08} & 1.3e+09 $\pm$ 1.7e+08 & 1.3e+09 $\pm$ 1.0e+08 & \textcolor{red}{2.5e+09 $\pm$ 2.0e+08} & \underline{1.1e+09 $\pm$ 1.1e+08} & 1.1e+09 $\pm$ 1.1e+08 \\
naval\textunderscore propulsion & 1.0e-08 $\pm$ 1.2e-10 & 1.0e-08 $\pm$ 1.2e-10 & \textbf{9.9e-09 $\pm$ 1.5e-10} & \textcolor{red}{1.4e-08 $\pm$ 3.5e-10} & \underline{9.9e-09 $\pm$ 9.8e-11} & 1.0e-08 $\pm$ 1.2e-10 & 1.0e-08 $\pm$ 1.2e-10 \\
parkinsons & 1.410 $\pm$ 0.156 & \textcolor{red}{2.574 $\pm$ 0.178} & 1.621 $\pm$ 0.143 & \textcolor{red}{3.587 $\pm$ 0.526} & \textcolor{red}{2.026 $\pm$ 0.173} & \underline{1.358 $\pm$ 0.119} & \textbf{1.351 $\pm$ 0.120} \\
powerplant & \textbf{1.911 $\pm$ 0.372} & 2.222 $\pm$ 0.307 & 2.015 $\pm$ 0.350 & 2.012 $\pm$ 0.374 & 2.024 $\pm$ 0.330 & 1.951 $\pm$ 0.363 & \underline{1.939 $\pm$ 0.363} \\
qsar & 0.110 $\pm$ 0.028 & \textcolor{red}{0.171 $\pm$ 0.023} & 0.113 $\pm$ 0.027 & 0.124 $\pm$ 0.029 & 0.125 $\pm$ 0.029 & \underline{0.109 $\pm$ 0.027} & \textbf{0.109 $\pm$ 0.027} \\
sulfur & \textbf{3.0e-04 $\pm$ 1.1e-04} & \underline{3.0e-04 $\pm$ 5.5e-05} & 3.4e-04 $\pm$ 8.9e-05 & \textcolor{red}{4.4e-04 $\pm$ 1.6e-04} & \textcolor{red}{6.4e-04 $\pm$ 1.2e-04} & 3.1e-04 $\pm$ 1.1e-04 & 3.1e-04 $\pm$ 1.1e-04 \\
superconductor & 13.708 $\pm$ 1.107 & 17.148 $\pm$ 1.369 & \textbf{13.069 $\pm$ 1.277} & \textcolor{red}{24.063 $\pm$ 2.010} & \textcolor{red}{22.872 $\pm$ 1.775} & \underline{13.663 $\pm$ 1.143} & 13.772 $\pm$ 1.182 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/a/table-combined-95-gamma-lambda-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (a) CLEAR calibration parameters $\lambda$ and $\gamma_1$ for 95\% prediction intervals across 10 seeds. Using all available variables. Showing median [min:max] values.}
\label{tab:combined_gamma_lambda_95_final_standard_variant_a}
\small
\begin{tabular}{lccc}
\toprule
Dataset & $\lambda$ & $\gamma_1$ \\
\midrule
ailerons & 0.95 [0.67:1.23] & 0.95 [0.82:1.06] \\
airfoil & 0.51 [0.20:1.40] & 1.29 [0.71:2.01] \\
allstate & 0.07 [0.00:0.95] & 1.75 [1.08:2.01] \\
ca\textunderscore housing & 0.54 [0.40:0.70] & 1.13 [1.02:1.30] \\
computer & 0.91 [0.15:2.65] & 1.09 [1.00:1.31] \\
concrete & 0.45 [0.18:18.47] & 1.61 [0.09:2.54] \\
elevator & 3.41 [2.55:5.02] & 1.17 [1.02:1.24] \\
energy\textunderscore efficiency & 0.08 [0.00:0.40] & 2.15 [1.45:2.92] \\
insurance & 0.31 [0.05:0.65] & 1.22 [0.94:1.55] \\
kin8nm & 1.18 [0.72:1.66] & 0.98 [0.78:1.24] \\
miami\textunderscore housing & 0.56 [0.35:2.16] & 1.14 [0.56:1.27] \\
naval\textunderscore propulsion & 1.48 [0.69:2.32] & 1.16 [1.05:1.28] \\
parkinsons & 1.49 [0.81:1.97] & 0.73 [0.63:0.89] \\
powerplant & 1.58 [1.16:4.63] & 0.74 [0.38:0.89] \\
qsar & 0.99 [0.50:1.68] & 0.98 [0.78:1.34] \\
sulfur & 0.73 [0.27:1.17] & 1.15 [1.05:1.45] \\
superconductor & 0.54 [0.36:0.96] & 1.05 [0.92:1.17] \\
\bottomrule
\end{tabular}
\end{table}

==> tex_tbls/pcs_cqr/standard/a/table-combined-95-mpiw-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (a) MPIW at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_mpiw_95_final_standard_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & 5.8e-04 $\pm$ 9.3e-06 & 6.2e-04 $\pm$ 8.7e-06 & 5.8e-04 $\pm$ 1.1e-05 & 6.4e-04 $\pm$ 1.3e-05 & 6.6e-04 $\pm$ 2.2e-05 & \underline{5.8e-04 $\pm$ 9.4e-06} & \textbf{5.8e-04 $\pm$ 9.1e-06} \\
airfoil & 7.101 $\pm$ 0.481 & \textcolor{red}{12.540 $\pm$ 0.481} & 7.380 $\pm$ 0.683 & 7.357 $\pm$ 0.425 & 8.417 $\pm$ 0.955 & \textbf{7.023 $\pm$ 0.459} & \underline{7.037 $\pm$ 0.458} \\
allstate & 6.4e+03 $\pm$ 3.8e+02 & 6.6e+03 $\pm$ 2.7e+02 & 6.4e+03 $\pm$ 3.0e+02 & 6.4e+03 $\pm$ 4.1e+02 & 8.0e+03 $\pm$ 2.9e+02 & \textbf{6.1e+03 $\pm$ 3.0e+02} & \underline{6.1e+03 $\pm$ 2.8e+02} \\
ca\textunderscore housing & 1.6e+05 $\pm$ 4.5e+03 & \textcolor{red}{3.7e+05 $\pm$ 1.2e+03} & 1.7e+05 $\pm$ 3.9e+03 & 1.7e+05 $\pm$ 5.8e+03 & 2.1e+05 $\pm$ 1.0e+04 & \underline{1.6e+05 $\pm$ 3.5e+03} & \textbf{1.6e+05 $\pm$ 4.1e+03} \\
computer & \underline{9.020 $\pm$ 0.752} & 9.805 $\pm$ 0.121 & 9.049 $\pm$ 0.996 & \textcolor{red}{1.8e+03 $\pm$ 1.2e+03} & 11.382 $\pm$ 0.706 & \textbf{8.990 $\pm$ 0.984} & 9.047 $\pm$ 0.706 \\
concrete & \textbf{18.917 $\pm$ 1.985} & \textcolor{red}{36.875 $\pm$ 2.073} & 20.130 $\pm$ 2.301 & \underline{18.918 $\pm$ 1.299} & 19.975 $\pm$ 2.229 & 19.049 $\pm$ 1.797 & 19.163 $\pm$ 1.907 \\
elevator & 9.6e-03 $\pm$ 1.5e-04 & \underline{8.9e-03 $\pm$ 1.4e-04} & 9.3e-03 $\pm$ 1.0e-04 & 0.011 $\pm$ 0.000 & \textbf{8.9e-03 $\pm$ 1.9e-04} & 9.7e-03 $\pm$ 1.7e-04 & 9.9e-03 $\pm$ 1.1e-04 \\
energy\textunderscore efficiency & \textbf{1.713 $\pm$ 0.193} & \textcolor{red}{7.732 $\pm$ 0.565} & \underline{1.833 $\pm$ 0.259} & 2.249 $\pm$ 0.231 & 2.265 $\pm$ 0.469 & 1.874 $\pm$ 0.165 & 1.926 $\pm$ 0.160 \\
insurance & \underline{1.8e+04 $\pm$ 1.6e+03} & 1.9e+04 $\pm$ 2.9e+03 & 1.9e+04 $\pm$ 3.1e+03 & \textcolor{red}{3.3e+04 $\pm$ 1.0e+04} & \textcolor{red}{2.7e+04 $\pm$ 4.7e+03} & 1.9e+04 $\pm$ 4.0e+03 & \textbf{1.7e+04 $\pm$ 2.4e+03} \\
kin8nm & 0.496 $\pm$ 0.007 & \textcolor{red}{0.676 $\pm$ 0.013} & 0.516 $\pm$ 0.010 & 0.515 $\pm$ 0.007 & 0.548 $\pm$ 0.015 & \textbf{0.496 $\pm$ 0.006} & \underline{0.496 $\pm$ 0.006} \\
miami\textunderscore housing & \underline{2.2e+05 $\pm$ 4.9e+03} & 2.7e+05 $\pm$ 2.1e+03 & 2.2e+05 $\pm$ 8.8e+03 & 2.5e+05 $\pm$ 6.8e+03 & \textcolor{red}{3.2e+05 $\pm$ 1.6e+04} & \textbf{2.2e+05 $\pm$ 4.2e+03} & 2.2e+05 $\pm$ 4.8e+03 \\
naval\textunderscore propulsion & 1.1e-03 $\pm$ 1.0e-05 & 1.1e-03 $\pm$ 1.1e-05 & \underline{1.1e-03 $\pm$ 1.1e-05} & 1.3e-03 $\pm$ 2.3e-05 & \textbf{1.1e-03 $\pm$ 1.2e-05} & 1.1e-03 $\pm$ 9.4e-06 & 1.1e-03 $\pm$ 9.3e-06 \\
parkinsons & \underline{10.917 $\pm$ 0.486} & \textcolor{red}{15.391 $\pm$ 0.618} & 11.939 $\pm$ 0.654 & \textcolor{red}{14.996 $\pm$ 1.028} & \textcolor{red}{14.537 $\pm$ 1.054} & 10.949 $\pm$ 0.360 & \textbf{10.799 $\pm$ 0.402} \\
powerplant & \textbf{12.232 $\pm$ 0.274} & 14.097 $\pm$ 0.258 & 12.959 $\pm$ 0.354 & 12.799 $\pm$ 0.448 & 13.169 $\pm$ 0.170 & 12.447 $\pm$ 0.272 & \underline{12.383 $\pm$ 0.291} \\
qsar & 3.094 $\pm$ 0.095 & \textcolor{red}{4.156 $\pm$ 0.096} & 3.298 $\pm$ 0.073 & 3.302 $\pm$ 0.106 & 3.581 $\pm$ 0.071 & \underline{3.084 $\pm$ 0.098} & \textbf{3.084 $\pm$ 0.107} \\
sulfur & 0.099 $\pm$ 0.004 & 0.102 $\pm$ 0.003 & \textbf{0.098 $\pm$ 0.004} & 0.119 $\pm$ 0.009 & 0.111 $\pm$ 0.007 & \underline{0.098 $\pm$ 0.005} & 0.098 $\pm$ 0.005 \\
superconductor & 28.172 $\pm$ 0.513 & 33.637 $\pm$ 0.364 & 28.274 $\pm$ 0.879 & 35.692 $\pm$ 1.013 & \textcolor{red}{47.360 $\pm$ 1.229} & \underline{28.014 $\pm$ 0.542} & \textbf{27.945 $\pm$ 0.448} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/a/table-uncertainty-metrics-95_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (a) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_standard_variant_a}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.52 [0.37:0.67] \\
airfoil & 3.34 [1.79:5.21] & 3.27 [1.92:4.57] & 0.99 [0.37:2.55] \\
allstate & 5998.48 [3817.06:6934.43] & 290.08 [0.00:2453.18] & 0.05 [0.00:0.64] \\
ca\textunderscore housing & 125093.50 [114102.96:142310.10] & 37700.45 [29483.44:44992.88] & 0.30 [0.22:0.39] \\
computer & 6.45 [6.01:7.99] & 2.32 [0.51:4.34] & 0.39 [0.06:0.69] \\
concrete & 8.95 [0.46:14.83] & 9.72 [5.17:18.45] & 0.86 [0.35:39.80] \\
elevator & 0.01 [0.01:0.01] & 0.00 [0.00:0.00] & 0.36 [0.27:0.49] \\
energy\textunderscore efficiency & 1.37 [0.79:1.84] & 0.27 [0.00:1.01] & 0.20 [0.00:1.28] \\
insurance & 17202.81 [13913.56:18465.50] & 852.20 [121.93:3006.17] & 0.06 [0.01:0.21] \\
kin8nm & 0.21 [0.16:0.27] & 0.29 [0.23:0.33] & 1.38 [0.83:1.98] \\
miami\textunderscore housing & 132180.87 [63417.71:151909.51] & 89093.15 [58612.93:165948.64] & 0.67 [0.41:2.62] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.22 [0.10:0.34] \\
parkinsons & 6.17 [5.25:7.45] & 4.77 [3.22:5.83] & 0.77 [0.43:1.03] \\
powerplant & 6.02 [3.06:7.16] & 6.17 [5.18:8.97] & 0.99 [0.72:2.93] \\
qsar & 1.58 [1.24:2.20] & 1.39 [0.96:1.93] & 0.88 [0.44:1.52] \\
sulfur & 0.07 [0.06:0.09] & 0.03 [0.01:0.03] & 0.40 [0.15:0.52] \\
superconductor & 22.09 [19.63:24.78] & 5.44 [3.99:8.68] & 0.25 [0.16:0.44] \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/b/table-combined-95-crps-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (b) CRPS at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_crps_95_final_standard_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & \underline{8.6e-05 $\pm$ 7.9e-07} & 9.6e-05 $\pm$ 1.4e-06 & 8.7e-05 $\pm$ 9.6e-07 & 8.9e-05 $\pm$ 7.8e-07 & 9.1e-05 $\pm$ 1.2e-06 & 8.6e-05 $\pm$ 8.5e-07 & \textbf{8.6e-05 $\pm$ 8.2e-07} \\
airfoil & 1.083 $\pm$ 0.062 & \textcolor{red}{2.192 $\pm$ 0.084} & 1.075 $\pm$ 0.068 & 1.109 $\pm$ 0.061 & 1.135 $\pm$ 0.080 & \underline{1.072 $\pm$ 0.058} & \textbf{1.072 $\pm$ 0.058} \\
allstate & 1.1e+03 $\pm$ 31.229 & 1.2e+03 $\pm$ 29.844 & \underline{1.0e+03 $\pm$ 29.016} & 1.0e+03 $\pm$ 30.491 & 1.1e+03 $\pm$ 37.696 & \textbf{1.0e+03 $\pm$ 25.475} & 1.0e+03 $\pm$ 24.303 \\
ca\textunderscore housing & 2.6e+04 $\pm$ 4.2e+02 & \textcolor{red}{8.3e+04 $\pm$ 6.9e+02} & 2.6e+04 $\pm$ 3.1e+02 & \underline{2.5e+04 $\pm$ 3.9e+02} & 2.8e+04 $\pm$ 3.2e+02 & 2.5e+04 $\pm$ 3.3e+02 & \textbf{2.5e+04 $\pm$ 3.3e+02} \\
computer & \underline{1.559 $\pm$ 0.073} & \textcolor{red}{2.843 $\pm$ 0.646} & \textbf{1.541 $\pm$ 0.048} & 2.008 $\pm$ 0.112 & 1.565 $\pm$ 0.052 & 1.577 $\pm$ 0.062 & 1.603 $\pm$ 0.065 \\
concrete & 2.927 $\pm$ 0.259 & \textcolor{red}{6.393 $\pm$ 0.361} & \underline{2.844 $\pm$ 0.256} & 2.974 $\pm$ 0.228 & \textbf{2.827 $\pm$ 0.257} & 2.918 $\pm$ 0.236 & 2.922 $\pm$ 0.235 \\
elevator & 1.3e-03 $\pm$ 1.3e-05 & \textcolor{red}{1.8e-03 $\pm$ 2.5e-05} & 1.4e-03 $\pm$ 1.5e-05 & 1.5e-03 $\pm$ 2.6e-05 & 1.4e-03 $\pm$ 2.5e-05 & \underline{1.3e-03 $\pm$ 1.5e-05} & \textbf{1.3e-03 $\pm$ 1.5e-05} \\
energy\textunderscore efficiency & \underline{0.274 $\pm$ 0.029} & \textcolor{red}{1.842 $\pm$ 0.138} & \textbf{0.262 $\pm$ 0.022} & \textcolor{red}{0.371 $\pm$ 0.030} & 0.293 $\pm$ 0.031 & 0.304 $\pm$ 0.025 & 0.313 $\pm$ 0.023 \\
insurance & \textcolor{red}{5.2e+03 $\pm$ 7.0e+02} & 4.0e+03 $\pm$ 1.1e+02 & \underline{3.1e+03 $\pm$ 1.3e+02} & \textcolor{red}{4.1e+03 $\pm$ 1.2e+03} & \textbf{3.0e+03 $\pm$ 3.5e+02} & \textcolor{red}{4.2e+03 $\pm$ 5.9e+02} & \textcolor{red}{4.2e+03 $\pm$ 5.6e+02} \\
kin8nm & \underline{0.076 $\pm$ 0.001} & \textcolor{red}{0.111 $\pm$ 0.001} & 0.077 $\pm$ 0.001 & 0.077 $\pm$ 0.001 & 0.078 $\pm$ 0.001 & \textbf{0.076 $\pm$ 0.001} & 0.076 $\pm$ 0.001 \\
miami\textunderscore housing & 3.4e+04 $\pm$ 9.5e+02 & \textcolor{red}{4.6e+04 $\pm$ 1.3e+03} & 3.6e+04 $\pm$ 1.1e+03 & 3.6e+04 $\pm$ 9.2e+02 & 4.5e+04 $\pm$ 1.2e+03 & \textbf{3.4e+04 $\pm$ 9.5e+02} & \underline{3.4e+04 $\pm$ 9.5e+02} \\
naval\textunderscore propulsion & \textbf{5.0e-04 $\pm$ 1.9e-05} & \textcolor{red}{0.128 $\pm$ 0.002} & \underline{5.0e-04 $\pm$ 1.6e-05} & \textcolor{red}{1.9e-03 $\pm$ 1.2e-04} & 5.8e-04 $\pm$ 2.4e-05 & 6.0e-04 $\pm$ 2.0e-05 & \textcolor{red}{7.8e-04 $\pm$ 3.3e-05} \\
parkinsons & \underline{2.166 $\pm$ 0.048} & \textcolor{red}{4.454 $\pm$ 0.054} & \textbf{2.157 $\pm$ 0.053} & 2.422 $\pm$ 0.040 & 2.294 $\pm$ 0.044 & 2.175 $\pm$ 0.046 & 2.175 $\pm$ 0.044 \\
powerplant & \underline{1.938 $\pm$ 0.034} & 2.288 $\pm$ 0.032 & 1.979 $\pm$ 0.030 & 1.938 $\pm$ 0.033 & \textbf{1.918 $\pm$ 0.024} & 1.970 $\pm$ 0.031 & 1.962 $\pm$ 0.033 \\
qsar & 0.487 $\pm$ 0.008 & \textcolor{red}{0.717 $\pm$ 0.010} & 0.491 $\pm$ 0.010 & 0.503 $\pm$ 0.006 & 0.499 $\pm$ 0.010 & \textbf{0.485 $\pm$ 0.009} & \underline{0.485 $\pm$ 0.009} \\
sulfur & 0.017 $\pm$ 0.000 & 0.018 $\pm$ 0.000 & \textbf{0.016 $\pm$ 0.000} & 0.018 $\pm$ 0.000 & 0.018 $\pm$ 0.000 & \underline{0.016 $\pm$ 0.000} & 0.016 $\pm$ 0.000 \\
superconductor & \underline{5.285 $\pm$ 0.152} & \textcolor{red}{8.867 $\pm$ 0.152} & 5.386 $\pm$ 0.129 & 5.396 $\pm$ 0.133 & 6.402 $\pm$ 0.131 & 5.350 $\pm$ 0.120 & \textbf{5.250 $\pm$ 0.123} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/b/table-combined-95-expectileloss-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (b) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_expectileloss_95_final_standard_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & 3.3e-09 $\pm$ 1.0e-10 & 4.0e-09 $\pm$ 1.7e-10 & 3.4e-09 $\pm$ 1.6e-10 & 4.2e-09 $\pm$ 9.6e-11 & 4.1e-09 $\pm$ 2.4e-10 & \textbf{3.3e-09 $\pm$ 1.0e-10} & \underline{3.3e-09 $\pm$ 1.0e-10} \\
airfoil & 0.499 $\pm$ 0.071 & \textcolor{red}{1.507 $\pm$ 0.123} & 0.528 $\pm$ 0.111 & 0.557 $\pm$ 0.088 & \textcolor{red}{0.687 $\pm$ 0.166} & \textbf{0.491 $\pm$ 0.071} & \underline{0.492 $\pm$ 0.071} \\
allstate & 5.8e+05 $\pm$ 7.1e+04 & 6.8e+05 $\pm$ 9.2e+04 & 6.1e+05 $\pm$ 8.1e+04 & 6.2e+05 $\pm$ 7.4e+04 & \textcolor{red}{8.6e+05 $\pm$ 1.1e+05} & \textbf{5.6e+05 $\pm$ 7.1e+04} & \underline{5.6e+05 $\pm$ 7.0e+04} \\
ca\textunderscore housing & 3.2e+08 $\pm$ 6.5e+06 & \textcolor{red}{1.4e+09 $\pm$ 1.1e+07} & 3.3e+08 $\pm$ 7.0e+06 & 3.8e+08 $\pm$ 1.1e+07 & \textcolor{red}{4.6e+08 $\pm$ 9.8e+06} & \underline{3.2e+08 $\pm$ 6.9e+06} & \textbf{3.2e+08 $\pm$ 7.8e+06} \\
computer & \textbf{1.387 $\pm$ 0.244} & \textcolor{red}{5.256 $\pm$ 1.415} & 1.591 $\pm$ 0.253 & \textcolor{red}{4.428 $\pm$ 0.575} & \textcolor{red}{1.904 $\pm$ 0.301} & \underline{1.507 $\pm$ 0.179} & 1.667 $\pm$ 0.186 \\
concrete & 4.220 $\pm$ 0.866 & \textcolor{red}{13.021 $\pm$ 1.326} & 4.346 $\pm$ 0.984 & \textbf{4.149 $\pm$ 0.779} & 4.408 $\pm$ 1.056 & \underline{4.187 $\pm$ 0.833} & 4.221 $\pm$ 0.847 \\
elevator & \underline{8.1e-07 $\pm$ 3.7e-08} & \textcolor{red}{1.3e-06 $\pm$ 6.9e-08} & 9.1e-07 $\pm$ 5.3e-08 & \textcolor{red}{1.6e-06 $\pm$ 9.0e-08} & \textcolor{red}{1.3e-06 $\pm$ 1.0e-07} & \textbf{8.0e-07 $\pm$ 3.6e-08} & 8.2e-07 $\pm$ 3.5e-08 \\
energy\textunderscore efficiency & \underline{0.044 $\pm$ 0.012} & \textcolor{red}{0.838 $\pm$ 0.127} & \textbf{0.039 $\pm$ 0.011} & \textcolor{red}{0.079 $\pm$ 0.009} & 0.051 $\pm$ 0.013 & \textcolor{red}{0.053 $\pm$ 0.009} & \textcolor{red}{0.056 $\pm$ 0.008} \\
insurance & 5.0e+06 $\pm$ 9.8e+05 & 5.9e+06 $\pm$ 1.0e+06 & \textbf{4.5e+06 $\pm$ 7.4e+05} & \textcolor{red}{1.1e+07 $\pm$ 6.4e+06} & 6.0e+06 $\pm$ 1.2e+06 & 5.9e+06 $\pm$ 2.8e+06 & \underline{4.8e+06 $\pm$ 1.2e+06} \\
kin8nm & 2.2e-03 $\pm$ 5.4e-05 & \textcolor{red}{4.0e-03 $\pm$ 8.8e-05} & 2.3e-03 $\pm$ 8.0e-05 & 2.3e-03 $\pm$ 4.0e-05 & 2.5e-03 $\pm$ 1.0e-04 & \textbf{2.2e-03 $\pm$ 4.8e-05} & \underline{2.2e-03 $\pm$ 4.9e-05} \\
miami\textunderscore housing & \textbf{1.1e+09 $\pm$ 1.1e+08} & \textcolor{red}{1.8e+09 $\pm$ 1.7e+08} & 1.3e+09 $\pm$ 1.7e+08 & 1.3e+09 $\pm$ 1.0e+08 & \textcolor{red}{2.5e+09 $\pm$ 2.0e+08} & \underline{1.1e+09 $\pm$ 1.1e+08} & 1.1e+09 $\pm$ 1.1e+08 \\
naval\textunderscore propulsion & \textbf{1.4e-07 $\pm$ 1.8e-08} & \textcolor{red}{3.3e-03 $\pm$ 9.5e-05} & \underline{1.5e-07 $\pm$ 1.7e-08} & \textcolor{red}{4.1e-06 $\pm$ 4.4e-07} & \textcolor{red}{2.6e-07 $\pm$ 5.4e-08} & \textcolor{red}{2.3e-07 $\pm$ 2.3e-08} & \textcolor{red}{4.9e-07 $\pm$ 4.8e-08} \\
parkinsons & \textbf{1.782 $\pm$ 0.081} & \textcolor{red}{5.243 $\pm$ 0.128} & 1.893 $\pm$ 0.093 & 2.369 $\pm$ 0.128 & 2.349 $\pm$ 0.142 & 1.786 $\pm$ 0.081 & \underline{1.785 $\pm$ 0.077} \\
powerplant & \textbf{1.911 $\pm$ 0.372} & 2.222 $\pm$ 0.307 & 2.015 $\pm$ 0.350 & 2.012 $\pm$ 0.374 & 2.024 $\pm$ 0.330 & 1.951 $\pm$ 0.363 & \underline{1.939 $\pm$ 0.363} \\
qsar & 0.110 $\pm$ 0.027 & \textcolor{red}{0.171 $\pm$ 0.024} & 0.113 $\pm$ 0.027 & 0.126 $\pm$ 0.028 & 0.125 $\pm$ 0.029 & \underline{0.109 $\pm$ 0.027} & \textbf{0.109 $\pm$ 0.027} \\
sulfur & \textbf{2.6e-04 $\pm$ 3.9e-05} & 2.9e-04 $\pm$ 3.8e-05 & 3.2e-04 $\pm$ 5.4e-05 & \textcolor{red}{3.8e-04 $\pm$ 4.6e-05} & \textcolor{red}{6.3e-04 $\pm$ 1.2e-04} & 2.6e-04 $\pm$ 3.9e-05 & \underline{2.6e-04 $\pm$ 3.9e-05} \\
superconductor & \underline{15.642 $\pm$ 1.475} & \textcolor{red}{27.189 $\pm$ 1.325} & 15.717 $\pm$ 1.336 & 19.710 $\pm$ 1.717 & \textcolor{red}{24.696 $\pm$ 1.602} & 15.977 $\pm$ 1.319 & \textbf{15.399 $\pm$ 1.377} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/b/table-combined-95-gamma-lambda-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (b) CLEAR calibration parameters $\lambda$ and $\gamma_1$ for 95\% prediction intervals across 10 seeds. Using all available variables. Showing median [min:max] values.}
\label{tab:combined_gamma_lambda_95_final_standard_variant_b}
\small
\begin{tabular}{lccc}
\toprule
Dataset & $\lambda$ & $\gamma_1$ \\
\midrule
ailerons & 0.95 [0.67:1.23] & 0.95 [0.82:1.06] \\
airfoil & 0.51 [0.20:1.40] & 1.29 [0.71:2.01] \\
allstate & 0.19 [0.00:1.22] & 1.68 [0.93:1.91] \\
ca\textunderscore housing & 0.54 [0.40:0.70] & 1.13 [1.02:1.30] \\
computer & 0.49 [0.32:0.88] & 1.18 [0.96:1.38] \\
concrete & 0.45 [0.18:18.47] & 1.61 [0.09:2.54] \\
elevator & 0.55 [0.41:0.85] & 1.09 [0.96:1.21] \\
energy\textunderscore efficiency & 0.08 [0.00:0.40] & 2.15 [1.45:2.92] \\
insurance & 0.21 [0.09:0.49] & 1.95 [1.24:2.82] \\
kin8nm & 1.18 [0.72:1.66] & 0.98 [0.78:1.24] \\
miami\textunderscore housing & 0.56 [0.35:2.16] & 1.14 [0.56:1.27] \\
naval\textunderscore propulsion & 0.01 [0.00:0.04] & 1.98 [1.66:2.35] \\
parkinsons & 0.71 [0.53:0.93] & 1.15 [1.03:1.31] \\
powerplant & 1.58 [1.16:4.63] & 0.74 [0.38:0.89] \\
qsar & 0.94 [0.53:1.91] & 1.02 [0.73:1.33] \\
sulfur & 0.57 [0.26:0.96] & 1.24 [1.05:1.49] \\
superconductor & 0.85 [0.56:1.43] & 0.90 [0.74:1.00] \\
\bottomrule
\end{tabular}
\end{table}

==> tex_tbls/pcs_cqr/standard/b/table-combined-95-mpiw-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (b) MPIW at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_mpiw_95_final_standard_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & 5.8e-04 $\pm$ 9.3e-06 & 6.2e-04 $\pm$ 8.7e-06 & 5.8e-04 $\pm$ 1.1e-05 & 6.4e-04 $\pm$ 1.3e-05 & 6.6e-04 $\pm$ 2.2e-05 & \underline{5.8e-04 $\pm$ 9.4e-06} & \textbf{5.8e-04 $\pm$ 9.1e-06} \\
airfoil & 7.101 $\pm$ 0.481 & \textcolor{red}{12.540 $\pm$ 0.481} & 7.380 $\pm$ 0.683 & 7.357 $\pm$ 0.425 & 8.417 $\pm$ 0.955 & \textbf{7.023 $\pm$ 0.459} & \underline{7.037 $\pm$ 0.458} \\
allstate & 6.3e+03 $\pm$ 2.4e+02 & 6.5e+03 $\pm$ 3.3e+02 & 6.4e+03 $\pm$ 3.5e+02 & 6.4e+03 $\pm$ 3.2e+02 & \textcolor{red}{8.0e+03 $\pm$ 3.4e+02} & \textbf{6.0e+03 $\pm$ 1.9e+02} & \underline{6.0e+03 $\pm$ 2.1e+02} \\
ca\textunderscore housing & 1.6e+05 $\pm$ 4.5e+03 & \textcolor{red}{3.7e+05 $\pm$ 1.2e+03} & 1.7e+05 $\pm$ 3.9e+03 & 1.7e+05 $\pm$ 5.8e+03 & 2.1e+05 $\pm$ 1.0e+04 & \underline{1.6e+05 $\pm$ 3.5e+03} & \textbf{1.6e+05 $\pm$ 4.1e+03} \\
computer & \textbf{9.833 $\pm$ 0.565} & \textcolor{red}{14.171 $\pm$ 2.903} & 10.335 $\pm$ 0.509 & \textcolor{red}{14.082 $\pm$ 0.842} & 11.152 $\pm$ 0.574 & \underline{10.020 $\pm$ 0.489} & 10.278 $\pm$ 0.470 \\
concrete & \textbf{18.917 $\pm$ 1.985} & \textcolor{red}{36.875 $\pm$ 2.073} & 20.130 $\pm$ 2.301 & \underline{18.918 $\pm$ 1.299} & 19.975 $\pm$ 2.229 & 19.049 $\pm$ 1.797 & 19.163 $\pm$ 1.907 \\
elevator & 8.5e-03 $\pm$ 1.2e-04 & 0.011 $\pm$ 0.000 & 9.0e-03 $\pm$ 2.3e-04 & \textcolor{red}{0.012 $\pm$ 0.000} & 0.010 $\pm$ 0.000 & \textbf{8.4e-03 $\pm$ 1.2e-04} & \underline{8.5e-03 $\pm$ 1.1e-04} \\
energy\textunderscore efficiency & \textbf{1.713 $\pm$ 0.193} & \textcolor{red}{7.732 $\pm$ 0.565} & \underline{1.833 $\pm$ 0.259} & 2.249 $\pm$ 0.231 & 2.265 $\pm$ 0.469 & 1.874 $\pm$ 0.165 & 1.926 $\pm$ 0.160 \\
insurance & \underline{1.9e+04 $\pm$ 2.6e+03} & \textcolor{red}{2.3e+04 $\pm$ 4.1e+03} & 2.2e+04 $\pm$ 3.9e+03 & \textcolor{red}{2.5e+04 $\pm$ 1.0e+04} & \textcolor{red}{2.7e+04 $\pm$ 4.4e+03} & 1.9e+04 $\pm$ 6.3e+03 & \textbf{1.8e+04 $\pm$ 3.8e+03} \\
kin8nm & 0.496 $\pm$ 0.007 & \textcolor{red}{0.676 $\pm$ 0.013} & 0.516 $\pm$ 0.010 & 0.515 $\pm$ 0.007 & 0.548 $\pm$ 0.015 & \textbf{0.496 $\pm$ 0.006} & \underline{0.496 $\pm$ 0.006} \\
miami\textunderscore housing & \underline{2.2e+05 $\pm$ 4.9e+03} & 2.7e+05 $\pm$ 2.1e+03 & 2.2e+05 $\pm$ 8.8e+03 & 2.5e+05 $\pm$ 6.8e+03 & \textcolor{red}{3.2e+05 $\pm$ 1.6e+04} & \textbf{2.2e+05 $\pm$ 4.2e+03} & 2.2e+05 $\pm$ 4.8e+03 \\
naval\textunderscore propulsion & \textbf{3.3e-03 $\pm$ 1.3e-04} & \textcolor{red}{0.391 $\pm$ 0.006} & \underline{3.4e-03 $\pm$ 1.7e-04} & \textcolor{red}{0.014 $\pm$ 0.001} & 4.3e-03 $\pm$ 2.6e-04 & 3.8e-03 $\pm$ 1.4e-04 & \textcolor{red}{4.9e-03 $\pm$ 2.3e-04} \\
parkinsons & \textbf{13.507 $\pm$ 0.448} & \textcolor{red}{23.175 $\pm$ 0.307} & 14.480 $\pm$ 0.584 & 15.576 $\pm$ 0.526 & 16.568 $\pm$ 0.539 & 13.511 $\pm$ 0.451 & \underline{13.508 $\pm$ 0.417} \\
powerplant & \textbf{12.232 $\pm$ 0.274} & 14.097 $\pm$ 0.258 & 12.959 $\pm$ 0.354 & 12.799 $\pm$ 0.448 & 13.169 $\pm$ 0.170 & 12.447 $\pm$ 0.272 & \underline{12.383 $\pm$ 0.291} \\
qsar & 3.114 $\pm$ 0.100 & \textcolor{red}{4.155 $\pm$ 0.096} & 3.308 $\pm$ 0.090 & 3.339 $\pm$ 0.141 & 3.594 $\pm$ 0.071 & \underline{3.090 $\pm$ 0.096} & \textbf{3.088 $\pm$ 0.091} \\
sulfur & 0.098 $\pm$ 0.003 & 0.100 $\pm$ 0.002 & 0.097 $\pm$ 0.004 & 0.117 $\pm$ 0.005 & 0.111 $\pm$ 0.007 & \textbf{0.097 $\pm$ 0.003} & \underline{0.097 $\pm$ 0.003} \\
superconductor & \underline{31.534 $\pm$ 0.797} & \textcolor{red}{44.546 $\pm$ 0.427} & 32.916 $\pm$ 0.652 & 35.037 $\pm$ 0.807 & \textcolor{red}{50.973 $\pm$ 0.957} & 32.120 $\pm$ 0.517 & \textbf{31.067 $\pm$ 0.602} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/b/table-uncertainty-metrics-95_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (b) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_standard_variant_b}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.52 [0.37:0.67] \\
airfoil & 3.34 [1.79:5.21] & 3.27 [1.92:4.57] & 0.99 [0.37:2.55] \\
allstate & 5740.13 [3217.88:6746.86] & 672.63 [0.00:2394.38] & 0.12 [0.00:0.74] \\
ca\textunderscore housing & 125093.50 [114102.96:142310.10] & 37700.45 [29483.44:44992.88] & 0.30 [0.22:0.39] \\
computer & 5.60 [4.65:6.52] & 4.11 [3.11:5.95] & 0.74 [0.48:1.28] \\
concrete & 8.95 [0.46:14.83] & 9.72 [5.17:18.45] & 0.86 [0.35:39.80] \\
elevator & 0.01 [0.01:0.01] & 0.00 [0.00:0.00] & 0.37 [0.28:0.56] \\
energy\textunderscore efficiency & 1.37 [0.79:1.84] & 0.27 [0.00:1.01] & 0.20 [0.00:1.28] \\
insurance & 16250.73 [10180.02:20632.47] & 2521.53 [1463.10:3967.20] & 0.16 [0.07:0.39] \\
kin8nm & 0.21 [0.16:0.27] & 0.29 [0.23:0.33] & 1.38 [0.83:1.98] \\
miami\textunderscore housing & 132180.87 [63417.71:151909.51] & 89093.15 [58612.93:165948.64] & 0.67 [0.41:2.62] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.10 [0.00:0.38] \\
parkinsons & 7.46 [6.78:8.56] & 5.71 [4.73:7.22] & 0.75 [0.56:1.01] \\
powerplant & 6.02 [3.06:7.16] & 6.17 [5.18:8.97] & 0.99 [0.72:2.93] \\
qsar & 1.63 [1.17:2.20] & 1.35 [0.99:2.00] & 0.83 [0.45:1.71] \\
sulfur & 0.07 [0.06:0.09] & 0.02 [0.01:0.03] & 0.32 [0.15:0.52] \\
superconductor & 22.16 [18.62:24.87] & 9.53 [7.07:13.38] & 0.43 [0.29:0.72] \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/c/table-combined-95-crps-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (c) CRPS at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_crps_95_final_standard_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & \underline{9.2e-05 $\pm$ 1.8e-06} & 9.9e-05 $\pm$ 1.6e-06 & \textbf{9.2e-05 $\pm$ 2.1e-06} & 9.7e-05 $\pm$ 2.0e-06 & 9.6e-05 $\pm$ 1.8e-06 & 9.2e-05 $\pm$ 1.9e-06 & 9.2e-05 $\pm$ 2.1e-06 \\
airfoil & 0.997 $\pm$ 0.080 & 1.263 $\pm$ 0.057 & \underline{0.982 $\pm$ 0.084} & 1.043 $\pm$ 0.079 & \textbf{0.974 $\pm$ 0.081} & 1.022 $\pm$ 0.085 & 1.009 $\pm$ 0.079 \\
allstate & 1.1e+03 $\pm$ 64.894 & 1.3e+03 $\pm$ 46.001 & 1.1e+03 $\pm$ 39.718 & 1.1e+03 $\pm$ 40.516 & \textbf{1.1e+03 $\pm$ 25.262} & 1.1e+03 $\pm$ 56.522 & \underline{1.1e+03 $\pm$ 50.665} \\
ca\textunderscore housing & 2.3e+04 $\pm$ 3.3e+02 & \textcolor{red}{3.1e+04 $\pm$ 4.4e+02} & 2.4e+04 $\pm$ 3.0e+02 & 2.4e+04 $\pm$ 3.9e+02 & 2.6e+04 $\pm$ 3.2e+02 & \underline{2.3e+04 $\pm$ 3.0e+02} & \textbf{2.3e+04 $\pm$ 3.1e+02} \\
computer & 1.218 $\pm$ 0.061 & 1.441 $\pm$ 0.047 & 1.249 $\pm$ 0.040 & 1.249 $\pm$ 0.079 & 1.264 $\pm$ 0.065 & \underline{1.209 $\pm$ 0.061} & \textbf{1.205 $\pm$ 0.059} \\
concrete & 3.227 $\pm$ 0.280 & 3.227 $\pm$ 0.141 & \underline{2.838 $\pm$ 0.223} & 3.288 $\pm$ 0.286 & \textbf{2.820 $\pm$ 0.224} & 3.270 $\pm$ 0.277 & 3.258 $\pm$ 0.268 \\
elevator & \textbf{1.2e-03 $\pm$ 1.1e-05} & \textcolor{red}{1.8e-03 $\pm$ 2.3e-05} & 1.2e-03 $\pm$ 1.2e-05 & 1.3e-03 $\pm$ 1.7e-05 & 1.3e-03 $\pm$ 1.6e-05 & 1.2e-03 $\pm$ 9.8e-06 & \underline{1.2e-03 $\pm$ 1.0e-05} \\
energy\textunderscore efficiency & 0.249 $\pm$ 0.030 & \textcolor{red}{0.644 $\pm$ 0.029} & \underline{0.242 $\pm$ 0.029} & 0.279 $\pm$ 0.035 & \textbf{0.239 $\pm$ 0.028} & 0.278 $\pm$ 0.036 & 0.276 $\pm$ 0.035 \\
insurance & 3.8e+03 $\pm$ 6.1e+02 & \textcolor{red}{4.6e+03 $\pm$ 5.3e+02} & \textcolor{red}{4.0e+03 $\pm$ 1.1e+03} & \underline{3.5e+03 $\pm$ 6.0e+02} & \textbf{3.0e+03 $\pm$ 2.9e+02} & \textcolor{red}{4.5e+03 $\pm$ 1.0e+03} & \textcolor{red}{4.9e+03 $\pm$ 1.6e+03} \\
kin8nm & \textbf{0.067 $\pm$ 0.001} & 0.085 $\pm$ 0.002 & 0.067 $\pm$ 0.002 & \underline{0.067 $\pm$ 0.001} & 0.067 $\pm$ 0.002 & 0.067 $\pm$ 0.002 & 0.067 $\pm$ 0.002 \\
miami\textunderscore housing & 3.4e+04 $\pm$ 8.1e+02 & 4.1e+04 $\pm$ 1.1e+03 & 4.1e+04 $\pm$ 1.4e+03 & 3.4e+04 $\pm$ 9.5e+02 & 4.3e+04 $\pm$ 1.5e+03 & \textbf{3.3e+04 $\pm$ 9.6e+02} & \underline{3.3e+04 $\pm$ 9.7e+02} \\
naval\textunderscore propulsion & \textbf{4.2e-04 $\pm$ 7.7e-06} & \textcolor{red}{7.8e-04 $\pm$ 1.8e-05} & 4.3e-04 $\pm$ 8.0e-06 & 4.3e-04 $\pm$ 8.5e-06 & 4.4e-04 $\pm$ 5.9e-06 & \underline{4.2e-04 $\pm$ 8.2e-06} & 4.3e-04 $\pm$ 9.2e-06 \\
parkinsons & \underline{1.866 $\pm$ 0.042} & \textcolor{red}{3.032 $\pm$ 0.105} & 1.874 $\pm$ 0.029 & 1.943 $\pm$ 0.045 & 1.900 $\pm$ 0.025 & 1.879 $\pm$ 0.040 & \textbf{1.855 $\pm$ 0.041} \\
powerplant & 1.763 $\pm$ 0.028 & 1.937 $\pm$ 0.045 & \textbf{1.714 $\pm$ 0.032} & 1.893 $\pm$ 0.038 & \underline{1.733 $\pm$ 0.030} & 1.768 $\pm$ 0.032 & 1.760 $\pm$ 0.032 \\
qsar & \underline{0.454 $\pm$ 0.013} & \textcolor{red}{0.605 $\pm$ 0.014} & \textbf{0.450 $\pm$ 0.011} & 0.519 $\pm$ 0.017 & 0.466 $\pm$ 0.018 & 0.465 $\pm$ 0.009 & 0.458 $\pm$ 0.009 \\
sulfur & 0.017 $\pm$ 0.001 & 0.020 $\pm$ 0.001 & \textbf{0.016 $\pm$ 0.000} & 0.018 $\pm$ 0.001 & 0.016 $\pm$ 0.000 & 0.016 $\pm$ 0.000 & \underline{0.016 $\pm$ 0.000} \\
superconductor & 4.597 $\pm$ 0.132 & 6.071 $\pm$ 0.181 & 4.683 $\pm$ 0.122 & 5.177 $\pm$ 0.179 & 5.616 $\pm$ 0.198 & \underline{4.584 $\pm$ 0.135} & \textbf{4.582 $\pm$ 0.133} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/c/table-combined-95-expectileloss-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (c) Expectile Loss at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_expectileloss_95_final_standard_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & \underline{3.7e-09 $\pm$ 1.5e-10} & 4.4e-09 $\pm$ 9.1e-11 & \textbf{3.6e-09 $\pm$ 1.2e-10} & \textcolor{red}{5.2e-09 $\pm$ 5.9e-10} & 4.5e-09 $\pm$ 2.6e-10 & 3.8e-09 $\pm$ 1.5e-10 & 3.8e-09 $\pm$ 1.4e-10 \\
airfoil & \textbf{0.485 $\pm$ 0.110} & \textcolor{red}{0.839 $\pm$ 0.046} & 0.552 $\pm$ 0.152 & 0.523 $\pm$ 0.117 & 0.535 $\pm$ 0.149 & 0.512 $\pm$ 0.123 & \underline{0.498 $\pm$ 0.113} \\
allstate & 6.0e+05 $\pm$ 4.2e+04 & 6.9e+05 $\pm$ 5.8e+04 & 6.2e+05 $\pm$ 1.1e+05 & 7.5e+05 $\pm$ 8.9e+04 & \textcolor{red}{8.0e+05 $\pm$ 9.8e+04} & \underline{5.9e+05 $\pm$ 4.4e+04} & \textbf{5.8e+05 $\pm$ 4.7e+04} \\
ca\textunderscore housing & 2.9e+08 $\pm$ 1.3e+07 & \textcolor{red}{4.5e+08 $\pm$ 1.2e+07} & 3.3e+08 $\pm$ 1.1e+07 & 3.2e+08 $\pm$ 1.6e+07 & \textcolor{red}{4.0e+08 $\pm$ 1.2e+07} & \underline{2.9e+08 $\pm$ 1.1e+07} & \textbf{2.9e+08 $\pm$ 1.1e+07} \\
computer & 1.177 $\pm$ 0.662 & \textcolor{red}{1.587 $\pm$ 0.902} & 1.272 $\pm$ 0.767 & 1.279 $\pm$ 0.638 & 1.301 $\pm$ 0.747 & \underline{1.154 $\pm$ 0.666} & \textbf{1.142 $\pm$ 0.675} \\
concrete & 4.804 $\pm$ 0.906 & 5.329 $\pm$ 0.684 & 4.831 $\pm$ 1.317 & \underline{4.730 $\pm$ 1.014} & \textbf{4.716 $\pm$ 1.345} & 4.810 $\pm$ 1.012 & 4.892 $\pm$ 1.034 \\
elevator & 6.5e-07 $\pm$ 1.4e-08 & \textcolor{red}{1.4e-06 $\pm$ 1.7e-08} & 7.5e-07 $\pm$ 3.5e-08 & \textcolor{red}{9.3e-07 $\pm$ 3.2e-08} & 8.3e-07 $\pm$ 3.6e-08 & \underline{6.5e-07 $\pm$ 1.4e-08} & \textbf{6.5e-07 $\pm$ 1.5e-08} \\
energy\textunderscore efficiency & \textbf{0.040 $\pm$ 0.019} & \textcolor{red}{0.280 $\pm$ 0.024} & 0.048 $\pm$ 0.036 & \textcolor{red}{0.056 $\pm$ 0.021} & \underline{0.047 $\pm$ 0.036} & \textcolor{red}{0.055 $\pm$ 0.021} & \textcolor{red}{0.055 $\pm$ 0.022} \\
insurance & 6.8e+06 $\pm$ 2.9e+06 & 6.1e+06 $\pm$ 5.1e+05 & \underline{6.0e+06 $\pm$ 9.0e+05} & \textcolor{red}{6.9e+06 $\pm$ 2.5e+06} & \textbf{5.2e+06 $\pm$ 1.2e+06} & \textcolor{red}{7.9e+06 $\pm$ 2.9e+06} & \textcolor{red}{9.0e+06 $\pm$ 2.9e+06} \\
kin8nm & \textbf{1.7e-03 $\pm$ 7.3e-05} & \textcolor{red}{2.8e-03 $\pm$ 8.4e-05} & 1.8e-03 $\pm$ 8.7e-05 & 1.8e-03 $\pm$ 7.6e-05 & 1.9e-03 $\pm$ 9.2e-05 & 1.8e-03 $\pm$ 7.8e-05 & \underline{1.8e-03 $\pm$ 7.7e-05} \\
miami\textunderscore housing & 1.1e+09 $\pm$ 6.9e+07 & \textcolor{red}{1.6e+09 $\pm$ 8.7e+07} & \textcolor{red}{2.0e+09 $\pm$ 2.2e+08} & 1.2e+09 $\pm$ 9.2e+07 & \textcolor{red}{2.1e+09 $\pm$ 2.1e+08} & \textbf{9.8e+08 $\pm$ 1.1e+08} & \underline{9.8e+08 $\pm$ 1.1e+08} \\
naval\textunderscore propulsion & \underline{8.1e-08 $\pm$ 3.2e-09} & \textcolor{red}{7.1e-07 $\pm$ 3.8e-08} & 8.5e-08 $\pm$ 3.5e-09 & 1.0e-07 $\pm$ 6.6e-09 & \textcolor{red}{1.1e-07 $\pm$ 3.7e-09} & \textbf{7.8e-08 $\pm$ 2.5e-09} & 8.3e-08 $\pm$ 2.6e-09 \\
parkinsons & \underline{1.400 $\pm$ 0.045} & \textcolor{red}{3.252 $\pm$ 0.175} & 1.574 $\pm$ 0.069 & 1.524 $\pm$ 0.068 & 1.613 $\pm$ 0.068 & 1.418 $\pm$ 0.046 & \textbf{1.380 $\pm$ 0.038} \\
powerplant & \underline{1.771 $\pm$ 0.379} & 1.961 $\pm$ 0.353 & \textbf{1.769 $\pm$ 0.373} & 1.980 $\pm$ 0.350 & 1.778 $\pm$ 0.360 & 1.782 $\pm$ 0.378 & 1.775 $\pm$ 0.381 \\
qsar & \underline{0.103 $\pm$ 0.027} & \textcolor{red}{0.151 $\pm$ 0.025} & \textbf{0.102 $\pm$ 0.028} & \textcolor{red}{0.139 $\pm$ 0.023} & 0.113 $\pm$ 0.029 & 0.108 $\pm$ 0.025 & 0.104 $\pm$ 0.025 \\
sulfur & 2.2e-04 $\pm$ 1.5e-05 & 2.7e-04 $\pm$ 5.1e-05 & \textcolor{red}{3.6e-04 $\pm$ 5.0e-05} & 2.7e-04 $\pm$ 2.3e-05 & \textcolor{red}{4.0e-04 $\pm$ 5.3e-05} & \underline{2.1e-04 $\pm$ 2.2e-05} & \textbf{2.1e-04 $\pm$ 2.3e-05} \\
superconductor & 13.197 $\pm$ 1.496 & \textcolor{red}{18.508 $\pm$ 1.509} & 13.209 $\pm$ 1.468 & \textcolor{red}{19.158 $\pm$ 2.174} & \textcolor{red}{19.795 $\pm$ 1.922} & \underline{13.165 $\pm$ 1.588} & \textbf{13.123 $\pm$ 1.541} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/c/table-combined-95-mpiw-final_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (c) MPIW at 95\% prediction intervals, aggregated across 10 seeds.Values $\geq 100$ or $< 0.01$ are presented in scientific notation with 1 decimal place. \textbf{Bold} values (desirable) are the minimum for that dataset and metric, while the \underline{underlined} values indicate the second-best result. \textcolor{red}{Red} values are more than 33\% worse than the best result.}
\label{tab:combined_mpiw_95_final_standard_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & CLEAR & ALEATORIC & ALEATORIC-R & PCS-EPISTEMIC & Naive & $\gamma_1=1$ & $\lambda=1$ \\
\midrule
ailerons & \underline{6.2e-04 $\pm$ 1.1e-05} & 6.8e-04 $\pm$ 8.6e-06 & \textbf{6.1e-04 $\pm$ 1.5e-05} & 7.1e-04 $\pm$ 4.2e-05 & 6.9e-04 $\pm$ 2.6e-05 & 6.2e-04 $\pm$ 1.0e-05 & 6.2e-04 $\pm$ 1.4e-05 \\
airfoil & \textbf{6.822 $\pm$ 0.602} & \textcolor{red}{9.769 $\pm$ 0.374} & 7.629 $\pm$ 0.856 & 6.996 $\pm$ 0.792 & 7.328 $\pm$ 0.819 & 7.031 $\pm$ 0.799 & \underline{6.915 $\pm$ 0.682} \\
allstate & 6.8e+03 $\pm$ 2.9e+02 & 7.7e+03 $\pm$ 3.3e+02 & 6.8e+03 $\pm$ 5.3e+02 & 7.3e+03 $\pm$ 5.5e+02 & 7.7e+03 $\pm$ 3.1e+02 & \underline{6.7e+03 $\pm$ 2.8e+02} & \textbf{6.7e+03 $\pm$ 2.7e+02} \\
ca\textunderscore housing & 1.5e+05 $\pm$ 5.3e+03 & \textcolor{red}{2.0e+05 $\pm$ 2.0e+03} & 1.7e+05 $\pm$ 7.0e+03 & 1.6e+05 $\pm$ 5.7e+03 & 1.9e+05 $\pm$ 8.6e+03 & \underline{1.5e+05 $\pm$ 4.4e+03} & \textbf{1.5e+05 $\pm$ 4.5e+03} \\
computer & 7.954 $\pm$ 0.388 & 10.142 $\pm$ 0.125 & 8.798 $\pm$ 0.351 & 8.322 $\pm$ 0.399 & 8.994 $\pm$ 0.616 & \underline{7.805 $\pm$ 0.385} & \textbf{7.737 $\pm$ 0.391} \\
concrete & 21.075 $\pm$ 2.217 & 23.851 $\pm$ 1.426 & 21.514 $\pm$ 2.139 & \textbf{20.742 $\pm$ 2.416} & \underline{20.936 $\pm$ 2.236} & 21.192 $\pm$ 2.281 & 21.317 $\pm$ 2.276 \\
elevator & 7.9e-03 $\pm$ 1.3e-04 & \textcolor{red}{0.012 $\pm$ 0.000} & 8.5e-03 $\pm$ 1.6e-04 & 9.4e-03 $\pm$ 1.7e-04 & 8.9e-03 $\pm$ 2.7e-04 & \underline{7.9e-03 $\pm$ 1.1e-04} & \textbf{7.9e-03 $\pm$ 9.6e-05} \\
energy\textunderscore efficiency & \textbf{1.577 $\pm$ 0.261} & \textcolor{red}{5.028 $\pm$ 0.241} & 1.843 $\pm$ 0.188 & \underline{1.654 $\pm$ 0.254} & 1.773 $\pm$ 0.184 & 1.695 $\pm$ 0.255 & 1.677 $\pm$ 0.261 \\
insurance & \underline{2.3e+04 $\pm$ 6.2e+03} & 2.4e+04 $\pm$ 1.4e+03 & 2.6e+04 $\pm$ 3.6e+03 & \textbf{2.3e+04 $\pm$ 6.0e+03} & 2.4e+04 $\pm$ 5.6e+03 & 2.5e+04 $\pm$ 5.6e+03 & 2.7e+04 $\pm$ 6.3e+03 \\
kin8nm & \textbf{0.448 $\pm$ 0.012} & 0.573 $\pm$ 0.015 & 0.456 $\pm$ 0.015 & 0.455 $\pm$ 0.011 & 0.474 $\pm$ 0.012 & 0.452 $\pm$ 0.014 & \underline{0.450 $\pm$ 0.013} \\
miami\textunderscore housing & 2.3e+05 $\pm$ 3.6e+03 & \textcolor{red}{2.9e+05 $\pm$ 5.1e+03} & \textcolor{red}{2.9e+05 $\pm$ 2.0e+04} & 2.4e+05 $\pm$ 6.1e+03 & \textcolor{red}{3.2e+05 $\pm$ 2.1e+04} & \textbf{2.0e+05 $\pm$ 5.6e+03} & \underline{2.0e+05 $\pm$ 5.7e+03} \\
naval\textunderscore propulsion & \underline{2.8e-03 $\pm$ 5.6e-05} & \textcolor{red}{7.2e-03 $\pm$ 1.6e-04} & 2.9e-03 $\pm$ 7.3e-05 & 3.1e-03 $\pm$ 9.7e-05 & 3.1e-03 $\pm$ 6.8e-05 & \textbf{2.8e-03 $\pm$ 3.3e-05} & 2.9e-03 $\pm$ 5.1e-05 \\
parkinsons & \underline{11.990 $\pm$ 0.335} & \textcolor{red}{17.828 $\pm$ 0.524} & 13.466 $\pm$ 0.512 & 12.459 $\pm$ 0.407 & 13.665 $\pm$ 0.471 & 12.061 $\pm$ 0.376 & \textbf{11.882 $\pm$ 0.346} \\
powerplant & \textbf{11.293 $\pm$ 0.302} & 12.624 $\pm$ 0.375 & 11.607 $\pm$ 0.320 & 12.140 $\pm$ 0.277 & 11.791 $\pm$ 0.259 & 11.357 $\pm$ 0.316 & \underline{11.344 $\pm$ 0.305} \\
qsar & \textbf{2.931 $\pm$ 0.130} & \textcolor{red}{3.964 $\pm$ 0.086} & 3.015 $\pm$ 0.110 & 3.383 $\pm$ 0.185 & 3.280 $\pm$ 0.172 & 2.992 $\pm$ 0.126 & \underline{2.939 $\pm$ 0.121} \\
sulfur & 0.101 $\pm$ 0.004 & 0.113 $\pm$ 0.004 & 0.099 $\pm$ 0.006 & 0.113 $\pm$ 0.003 & 0.104 $\pm$ 0.006 & \underline{0.096 $\pm$ 0.002} & \textbf{0.094 $\pm$ 0.003} \\
superconductor & 28.088 $\pm$ 0.812 & 36.044 $\pm$ 0.523 & 30.215 $\pm$ 1.595 & 33.859 $\pm$ 1.241 & \textcolor{red}{44.356 $\pm$ 1.361} & \underline{27.884 $\pm$ 0.914} & \textbf{27.881 $\pm$ 0.857} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tex_tbls/pcs_cqr/standard/c/table-uncertainty-metrics-95_standard.tex <==
\begin{table}[!htbp]
\centering
\caption{Variant (c) uncertainty metrics for 95\% prediction intervals across 10 seeds. Values are shown as median [min:max]. A = aleatoric uncertainty, E = epistemic uncertainty, E/A = uncertainty ratio.}
\label{tab:uncertainty_metrics_95_standard_variant_c}
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Dataset & \multicolumn{3}{c}{CLEAR} \\
\cmidrule(lr){2-4}
 & A & E & E/A \\
\midrule
ailerons & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 0.25 [0.06:0.51] \\
airfoil & 0.97 [0.16:2.57] & 5.98 [4.11:7.49] & 6.36 [1.79:37.39] \\
allstate & 6498.87 [258.62:7033.60] & 481.38 [0.00:6471.51] & 0.07 [0.00:25.02] \\
ca\textunderscore housing & 54584.22 [25576.43:72644.44] & 98858.11 [77798.20:123737.70] & 1.79 [1.07:4.84] \\
computer & 1.52 [0.45:5.11] & 6.26 [3.76:7.65] & 4.02 [0.74:17.03] \\
concrete & 1.45 [0.02:8.81] & 18.08 [11.18:24.47] & 12.98 [1.27:875.50] \\
elevator & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 1.06 [0.75:1.56] \\
energy\textunderscore efficiency & 0.52 [0.00:1.74] & 0.96 [0.25:2.14] & 2.10 [0.15:1522.04] \\
insurance & 2973.62 [11.07:9594.79] & 17334.72 [11463.50:27593.72] & 11.47 [1.32:1801.27] \\
kin8nm & 0.28 [0.21:0.30] & 0.16 [0.15:0.25] & 0.57 [0.50:1.15] \\
miami\textunderscore housing & 16740.85 [6466.44:23566.99] & 205362.95 [203073.16:228659.76] & 12.20 [9.05:35.36] \\
naval\textunderscore propulsion & 0.00 [0.00:0.00] & 0.00 [0.00:0.00] & 1.71 [1.32:2.23] \\
parkinsons & 2.64 [0.46:3.96] & 9.32 [8.39:11.51] & 3.47 [2.12:24.89] \\
powerplant & 5.05 [2.40:6.28] & 6.32 [5.33:8.95] & 1.22 [0.85:3.72] \\
qsar & 1.99 [0.91:2.45] & 1.08 [0.46:2.04] & 0.54 [0.19:2.23] \\
sulfur & 0.02 [0.01:0.03] & 0.08 [0.06:0.09] & 3.30 [2.08:9.34] \\
superconductor & 20.24 [12.55:25.36] & 8.68 [3.49:15.03] & 0.44 [0.14:1.15] \\
\bottomrule
\end{tabular}
}
\end{table}
